Invisible and Semi-invisible Decays of Bottom Baryons

The similar densities of dark matter and baryons in the universe imply that they might arise from the same ultraviolet model. The B-Mesogenesis, which assumes dark matter is charged under the baryon number, attempts to simultaneously explain the origin of baryon asymmetry and dark matter in the universe. In particular, the B-Mesogenesis might induce bottom-baryon decays into invisible or semi-invisible final states, which provide a distinctive signal for probing this scenario. In this work, we systematically study the invisible decays of bottom baryons into dark matters, and semi-invisible decays of bottom baryons into a meson or a photon together with a dark matter particle. In particular, the fully invisible decay can explore the stable particles in B-Mesogenesis. Some QCD-based frameworks are used to calculate the hadronic matrix elements under the B-Mesogenesis model. We estimate the constraints on the Wilson coefficients or the product of some new physics couplings with the Wilson coefficients by the semi-invisible and invisible decays of bottom baryons at future colliders.

==> 3-1-Calculation-invisible.tex <==


% \input{Feynman-diagram/invisible-decay-feynman}
% \input{Feynman-diagram/charged-baryon-decay-feynman}


\subsection{Fully invisible decay for $\Lambda_b^0$}
%Within the Lagrangian above, the Feynman diagrams of invisible decay $\Lambda_b\to\xi\phi$ are displayed in FIG. \ref{Fig:Baryon_invisible-decay}. 
%
%
\begin{figure}{}
    \centering
        \includegraphics[width=0.8\textwidth]{Fig/invisible-final-states-Li.eps}
\caption{The Feynman diagram for $\Lambda_b^0 \to \xi\bar{\phi}$ process, with the bold line denoting the $b$ quark.}
\label{FIG:Lambda_b_to_invisible}
\end{figure}
%
%
Under the B-Mesogenesis scenario, $\Lambda_b^0 \to \xi \bar{\phi}$ channel is governed by both effective operators ${\mathcal{O}}_{ud,b}^{'L,R}$ and ${\mathcal{O}}_{ub,d}^{'L,R}$. The Feynman diagram is shown in FIG. \ref{FIG:Lambda_b_to_invisible}. The decay amplitudes could be respectively expressed as
%
\begin{equation}{\label{Eq:amplitudes`invisible`decay}}
    \begin{aligned}
        i \mathcal{M}_{ud,b}^{L,R} &=
    y_dC^{L,R}_{ud,b} \bigg(\bar{u}_{\xi}^{\mathcal{C}}(q)
    \frac{\slashed{p}{'}+m_{\psi}}{p'^{2}-m_{\psi}^2}  
  \langle  0| \mathcal{O}^{'L,R}_{ud,b} |\Lambda_b^0(p{'}) \rangle \bigg), \\
     i \mathcal{M}_{ub,d}^{L,R} &=
    y_dC^{L,R}_{ub,d} 
    \bigg(\bar{u}_{\xi}^{\mathcal{C}}(q)
    \frac{\slashed{p}{'}+m_{\psi}}{p'^{2}-m_{\psi}^2}  
    \langle 0|   \mathcal{O}^{'L,R}_{ub,d} |\Lambda_b^0(p{'})\rangle \bigg),
    \end{aligned}
\end{equation}
%
where $u_{\xi}(q)$ is the spinor for $\xi$ with the four-momentum $q$. %and $\Lambda_b$ carries 4-momentum $p$. 
%The four-momentums are satisfying the on shell conditions $q^2 = m_{\xi}^2$ and $p^2 = m_{\Lambda_b}^2$.
%
To estimate the branching ratios of the invisible baryon decay, we have to firstly calculate the corresponding hadronic matrix elements in Eq. \eqref{Eq:amplitudes`invisible`decay}, which could be parameterized in terms of the coupling constants defined by
%
\begin{equation}{\label{our_coupling}}
   \begin{aligned}
        \langle 0| \mathcal{O}^{'L,R}_{ud,b}  |\Lambda_b^0(p{'})\rangle = \lambda_{ud,b}^{L,R}\ P_R u_{\Lambda_b}(p{'}),
        %
     \quad
    %
     \langle 0| \mathcal{O}^{'L,R}_{ub,d} |\Lambda_b^0(p{'})\rangle = \lambda_{ub,d}^{L,R}\ P_R u_{\Lambda_b}(p{'}).
   \end{aligned}
\end{equation}
%
We found that the  coupling $\lambda_{ud,b}^{L,R}$ and $\lambda_{ub,d}^{L,R}$ could be related to the coupling $f_{\Lambda_b}^{(1,2)}$ defined in Eq. \eqref{Eq:definition-decay-constants} by multiply corresponding matrix element. For instance,
\begin{equation}
\begin{aligned}
    \langle 0| \mathcal{O}^{'L,R}_{ud,b}  |\Lambda_b^0(p{'})\rangle  &=   \epsilon_{ijk} \langle 0|
  \left[u^{i T}\, C P_{L, R}\, d^j \right]b_{R}^k
  | \Lambda_b^0\left(p{'}\right) \rangle 
  \\
  &=\sum_{\rho} (CP_{L,R})^{\alpha\beta}(P_R)^{\rho\gamma} \left\{  \epsilon_{ijk} \langle 0| u^{iT}_{\alpha} d^{j}_{\beta} b^{k}_{\gamma} |\Lambda_b^0(p{'}) \rangle \right\}
  \\
  &= \frac{1}{4}\left\{ f^{(1)}_{\Lambda_b} \text{Tr}[CP_{L,R}\gamma_5C^T]+ f^{(2)}_{\Lambda_b}\text{Tr}[ CP_{L,R}\slashed{v}\gamma_5C^T ] \right\} P_R u_{\Lambda_b}(p{'}).
\end{aligned}
\end{equation}
%
%
The last line is the result after using Eq. \eqref{Eq:definition-decay-constants}. After the trace, we can obtain the relations,
\begin{equation}{\label{equ:InvisibleDecayConstant}}
    \begin{aligned}
        \lambda^L_{ud,b} &= -\frac{1}{2} f_{\Lambda_b}^{(1)}, \quad 
         \lambda^R_{ud,b} &= +\frac{1}{2} f_{\Lambda_b}^{(1)}.
    \end{aligned} 
\end{equation}
The same operation can be used for $\lambda^{L,R}_{ub,d}$, which can obtain,
%
\begin{equation}{\label{equ:InvisibleDecayConstant2}}
    \begin{aligned}
         \lambda^L_{ub,d} &= -\frac{1}{4} f_{\Lambda_b}^{(2)}, \quad
         \lambda^R_{ub,d} &= +\frac{1}{4} f_{\Lambda_b}^{(1)}.
    \end{aligned}
\end{equation}
%
%
% We found that the  coupling $\lambda_{ud,b}^{L,R}$ and $\lambda_{ub,d}^{L,R}$ could be related to the coupling $f_{\Lambda_b}^{(1,2)}$ defined in the heavy-quark limit  \cite{Grozin:1992td, Groote:1997yr, Ball:2008fw, Ali:2012pn, Bell:2013tfa} as
% %
% \begin{equation}\label{matrix-elements}
%       \begin{aligned}
%           \bra{0} \mathcal{J}_{\Lambda_b}^{(1,2)}(0) \ket{\Lambda_b\left(p\right)}\equiv & \ f_{\Lambda_b}^{(1,2)} \ u_{\Lambda_b}\left(p\right), \\
%           %
%           \mathcal{J}_{\Lambda_{b}}^{(1)}(x) = \epsilon_{ijk} \left[  u^{iT}(x) C \gamma_5 d^j(x) \right]  b^k(x),\quad &\mathcal{J}_{\Lambda_{b}}^{(2)}(x) = \epsilon_{ijk} \left[  u^{iT}(x) C \gamma_5 \slashed{v} d^j(x) \right]  b^k(x),
%       \end{aligned}
% \end{equation}
% %
% where the form of operators $\mathcal{J}_{\Lambda_b}^{(1,2)}$ are determined by the $P$ parity and the heavy quark symmetry, and $v^{\mu}$ is the four-speed of heavy quark.
% %
% Their relations are, {\color{red}(why?)}
% %
% \begin{equation}{\label{equ:InvisibleDecayConstant}}
%     \begin{aligned}
%         \lambda^L_{ud,b} &= -\frac{1}{2} f_{\Lambda_b}^{(1)}, \\
%          \lambda^R_{ud,b} &= +\frac{1}{2} f_{\Lambda_b}^{(1)},
%     \end{aligned} 
%     \quad
%     \begin{aligned}
%          \lambda^L_{ub,d} &= -\frac{1}{4} f_{\Lambda_b}^{(2)}, \\
%          \lambda^R_{ub,d} &= +\frac{1}{4} f_{\Lambda_b}^{(1)}.
%     \end{aligned}
% \end{equation}
%
For the numerical value of the couplings we quote the result of the NLO QCD sum rule
analysis in Ref. \cite{Groote:1997yr}:
%
\begin{equation}
f_{\Lambda_b}^{(2)}\approx f_{\Lambda_b}^{(1)} = 0.030 \pm 0.005 \ [\text{GeV}^3].
\end{equation}
%
Then, we could estimate the branching ratios of the invisible baryon decay. 
%
Assuming the new physics individually exist in either the left-handed or right-handed component, the branching ratios of $\Lambda_b\to\xi\bar{\phi}$ is  given by
%
\begin{equation}\label{eq_branching-ratio}
\begin{aligned}
\mathcal{BR}({\Lambda_b\to\xi\bar{\phi}})^{L,R}_{u_ad_b,d_c}
&=
\frac{\left|\Vec{q}_{\xi}\right|}{8 \pi m_{\Lambda_b} \Gamma_{\Lambda_b}} 
%
\bigg(\left|y_d\right|^2 \left|C^{L,R}_{u_ad_b,d_c}\right|^2
\left|\lambda_{_{u_ad_b,d_c}}^{L,R}\right|^2 \bigg)
%
\frac{E_{\xi}\left( m_{\Lambda_b}^2 + m^2_{\psi} \right) + 2 m_{\Lambda_b} m_{\psi}m_{\xi}}{\left(m_{\Lambda_b  }^2 -m_{\psi}^2\right)^2},
\end{aligned}
\end{equation}
%
where $(u_ad_b,d_c)$ represents $(ud,b)$ or $(ub,d)$ for different effective operators $ \mathcal{O}^{L,R}_{ud,b}$ and $ \mathcal{O}^{L,R}_{ub,d}$ convention in Eq. \eqref{Eq:Effective-Operators} respectively, $m_i~\!(i=\Lambda_b^0,\bar{\psi},\bar{\phi},\xi)$ and $\Gamma_{\Lambda_b}$ are the mass of particle $i$ and the total width of heavy baryons. 
The $\Vec{q}_{\xi}$ and $E_{\xi} = \frac{m_{\Lambda_b}^2  + m_{\xi}^2 - m_{\phi}^2}{2m_{\Lambda_b}}$ are the momentum and kinetic energy of $\xi$ in heavy baryon $\Lambda_b^0$ rest frame. 

% The coupling $\lambda_{\Lambda_b}^{L,R}$ could be related to the coupling $\lambda_{\Lambda_b}^{1,2}$ defined in the heavy-quark limit  \cite{Grozin:1992td, Groote:1997yr, Ball:2008fw, Ali:2012pn, Bell:2013tfa}, 
% \begin{equation}\label{matrix-elements}
%       \bra{0} \mathcal{J}_{\Lambda_b}^{1,2}(0) \ket{\Lambda_b\left(p\right)}\equiv\lambda_{\Lambda_b}^{1,2} \ u_{\Lambda_b}\left(p\right),
% \end{equation}
% where the current $\mathcal{J}_{\Lambda_b}$ for $\Lambda_b^0$ are respectively shown as,
% \begin{equation}{\label{currents}}
%     \begin{aligned}
%     \mathcal{J}_{\Lambda_{b}}^{1}(x) &= \epsilon_{ijk} \left[  u^{iT}(x) \mathcal{C} \gamma_5 d^j(x) \right]  b^k(x),\ \mathcal{J}_{\Lambda_{b}}^{2}(x) = \epsilon_{ijk} \left[  u^{iT}(x) \mathcal{C} \gamma_5 \slashed{v} d^j(x) \right]  b^k(x),
%     \end{aligned}
% \end{equation}
% whose form is determined by $P$ parity and the heavy quark symmetry, besides, the $\mathcal{C}$ is the charge conjugation matrix and $v^{\mu}$ is the four-speed of heavy quark. The relations between $\lambda_{\Lambda_b}^{L,R}$ and $\lambda_{\Lambda_b}^{1,2}$ are listed in the Table. \ref{tab:relation_coupling_constants}. For the numerical value of the couplings we quote the result of the NLO QCD sum rule
% analysis in Ref. \cite{Groote:1997yr}:
% \begin{equation}
% \lambda_{\Lambda_b}^{2}\approx\lambda_{\Lambda_b}^{1} = 0.030 \pm 0.005 \ [\text{GeV}^3]
% \end{equation}


% \begin{table}[]
%     \centering
%     \caption{The relation between the coupling $\lambda_{\Lambda_b}^{L,R}$ in \eqref{our_coupling} and standard baryon coupling constants $\lambda_{\Lambda_b}^{(1,2)}$ in \eqref{matrix-elements}.}
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%       $\mathcal{O}^{'L,R}_{u_ad_b,d_c}$   & \quad   $\mathcal{O}^{'L,R}_{ud,b}$ \quad &    \quad $\mathcal{O}^{'L,R}_{ub,d}$ \quad \tabularnewline
% \hline 
% \hline 
%        $\lambda_{\Lambda_b}^L$  & $-\frac{1}{2} \lambda_{\Lambda_b}^{1}$ & $-\frac{1}{4} \lambda_{\Lambda_b}^{2}$   \\
% \hline 
%        $\lambda_{\Lambda_b}^R$  & $\quad \frac{1}{2} \lambda_{\Lambda_b}^{1}$  & $ \quad \frac{1}{4} \lambda_{\Lambda_b}^{1}$ \\
%        \hline
%     \end{tabular}
%     \label{tab:relation_coupling_constants}
% \end{table}

==> 3-2-Calculation-Ppsi.tex <==
\subsection{Hadronic semi-invisible decays of $\Lambda_b/\Xi_b\to P \bar{\psi}$ }
\begin{figure}{}
    \centering
        \includegraphics[width=0.9\textwidth]{Fig/hadron-final-states-Li.eps}
\caption{ The Feynman diagrams of the $\Lambda_b^0/\Xi_b^- \to P\bar{\psi}$ decays, where the bold line represents the $b$ quark and the circle cross denotes the currents in the $\mathcal{O}^{L,R}$ operators.}
    \label{fig:hadron-final-states}
\end{figure}
In this subsection, we construct  the factorization formula and calculate the hadronic matrix elements of $\Lambda_b^0/\Xi_b^- \to P^{0,-}\bar{\psi}$   decays explicitly in the heavy quark limit. The relevant diagrams are shown in Fig. \ref{fig:hadron-final-states}. Using the effective Lagrangian given in Eq. \eqref{Eq:effective-Lagragian2}, one can express the
decay amplitude for the operator $\mathcal{O}^{'L,R}_{u_ad_b,d_c}$ as,
%
\begin{equation}{\label{Eq:baryon-meson-amplitude}}
     i \mathcal{M} =
C^{L,R}_{u_ad_b,d_c}
\bigg(
\bar{v}_{\psi}^{\mathcal{C}}(q)
    \langle P(p)|
    \mathcal{O}^{'L,R}_{u_ad_b,d_c} |\mathcal{B}(p')\rangle \bigg),
\end{equation}
%
where $v_{\psi}$ is the spinor of dark baryon $\bar{\psi}$ with momentum $q = p'-p$, and $\mathcal{B}$ represents $\Lambda_b^0$ or $\Xi_b^-$ with momentum $p'=m_{\mathcal{B}}v$. 
%
The hadronic matrix elements could be parameterized in terms of two form factors respectively,
%
\begin{equation}{\label{Eq:B-P-form`factors-def}}
    \begin{aligned}
          \langle P(p)|
    \mathcal{O}^{'L,R}_{u_ad_b,d_c} |\mathcal{B}(p')\rangle =  P_R \bigg( \frac{\slashed{p}'}{m_{\mathcal{B}}}\zeta^{\mathcal{B} \to P(L,R)}_1(q^2) + \frac{\slashed{q}}{m_{\mathcal{B}}} \zeta^{\mathcal{B} \to P(L,R)}_2(q^2) \bigg) u_{\mathcal{B}}(p').
    \end{aligned}
\end{equation}
%
%Considering a decay of heavy-flavor baryons into final-state light mesons $P$ and dark baryon field $\bar{\psi}$ with mass around 1 GeV, the final-state particles can be approximately regarded as being on the light-cone.
%Therefore, we could employ the method of QCD factorization to expand the decay amplitude to leading power and perform factorization analysis.
%光锥坐标系、 动量守恒、 重夸克极限 、 两个幂次压低的图。 
We will calculate the form factors working in the rest frame of the heavy baryon and choose two light-cone vectors along the fast-moving final state particles with the conventions of
\begin{equation}
n_\mu=(1,0,0,1),\quad \bar{n}_\mu=(1,0,0,-1),\quad v^\mu=(1,0,0,0).
\end{equation}
Then any 4-vector $p^{\mu}$ can be decomposed as light-cone components with a perpendicular component
\begin{equation}
    p^\mu=(n\cdot p)\frac{\bar{n}^\mu}{2}+(\bar{n}\cdot p)\frac{n^\mu}{2}+p_{\perp}^\mu\equiv (n\cdot p,\bar{n}\cdot p,p_{\perp}) .
\end{equation}
When computing the Feynman diagrams in the heavy quark limit, four different momentum configurations show up in the heavy-to-light process under consideration,
\begin{equation}
    \begin{aligned}
   & p'=(m_\mathcal{B},m_\mathcal{B},0) 
   \qquad \qquad \qquad \sim m_\mathcal{B}(1,1,0),\\
   & q=(m_\mathcal{B},\frac{m_{\psi}^2}{m_\mathcal{B}},0) \qquad \qquad \qquad \sim m_\mathcal{B}(1,\lambda^2,0),
        \\
 & p=(\frac{m^2_P}{\bar{n}\cdot p},m_\mathcal{B}-\frac{m_{\psi}^2}{m_\mathcal{B}},0)   \qquad \ \ \sim m_\mathcal{B}(\lambda^2,1,0), \\
 & k=(\Lambda_{\text{QCD}},\Lambda_{\text{QCD}},\Lambda_{\text{QCD}})\qquad  \sim m_\mathcal{B}(\lambda,\lambda,\lambda),
    \end{aligned}
\end{equation} 
where $k$ corresponds to the momentum of the light spectator quark in the baryon. The parameter $\lambda\sim\frac{m_{\psi}}{m_{\mathcal{B}}}\sim\frac{m_P}{m_\mathcal{B}}$, which is vanishing in the heavy quark limit, hence $\lambda=0$ is used in this work. Then the contribution of the second form factor $\zeta_{2}^{\mathcal{B}\to P (L,R)}$ in Eq. \eqref{Eq:B-P-form`factors-def} to the decay amplitudes in Eq. \eqref{Eq:baryon-meson-amplitude} vanishes, due to the equation of motion $\frac{\slashed{q}}{m_{\mathcal{B}}}v_{\psi}=\lambda v_{\psi}=0.$

When considering only the leading twist distribution amplitudes and the tree-level QCD calculations, the contribution of operator $\mathcal{O}^{'R}_{u_ad_b, d_b}$ in Eq. \eqref{Eq:effective-Lagragian2} to the transition matrix element always vanish, since there is an odd number of Dirac matrices between the two chiral projection matrices $P_R=\frac{1+\gamma_5}{2}$ within the operator $\mathcal{O}^{'R}_{u_ad_b, d_b}$. 
%
In the heavy quark limit, the transition amplitude in Eq.~\eqref{Eq:baryon-meson-amplitude} also vanishes for operators  $\mathcal{O}^{L}_{ud,b}$ and $\mathcal{O}^{L}_{us,b}$ due to the parity conservation. Take $\Lambda_b^0\to \pi^0 \bar{\psi}$ as an example, the partonic amplitude\footnote{The partonic amplitude defined as replacing $|\Lambda_b^0(p')\rangle$ and $\langle P(p)|$ by $|u(k_1) d(k_2) b(m_bv)\rangle$ and $\langle \bar{q} (xp) q(\bar{x}p)|$ \cite{Wang:2015vgv}.}
%$ \langle P(p')\bar{\psi}(q)| \mathcal{O}^{L}_{ud,b}|\Lambda_b(p)\rangle$ 
can be factorized as a product of two transition matrix elements in the spin space,
$i \mathcal{M}  
 \propto 
 \langle\bar{\psi}(q)|\,\bar{\psi}^{\mathcal{C}} b_R \, | b(m_bv)\rangle\,
 \langle \bar{q} (xp)q(\bar{x}p)| \,  \bar{u}^{\mathcal{C}}_L d_L \,|u(k_1) d(k_2)\rangle.$ Then we will find that there is a trace in the second matrix element in our calculation, which is always zero because there is an odd number of $\gamma$ matrices. 
 And we find that the $\gamma_5$ in the operator $\bar{u}^{\mathcal{C}}_L d_L$ cannot contribute to the trace, because there are only two independent Lorentz vectors in this process to contract with the 4-dimensional antisymmetric tensor $\epsilon_{\mu\nu\rho\sigma}$. Actually, the $J^P$ quantum number of quark pair $(ud)$ in $\Lambda_b^0$ baryon is $0^+$ in the leading twist approximation, and $\langle q (xp)\bar{q}(\bar{x}p)| \,  \bar{u}^{\mathcal{C}}_L d_L \,|u(k_1) d(k_2)\rangle$ describes a scalar decay into a pseudoscalar induced by a scalar operator, which violate parity conservation.
 The hadronic effects will not affect this conclusion cause the perturbative results in the final factorization formula are independent of the external state \cite{Descotes-Genon:2002crx}.

In the following
calculation, we only consider the contribution of the 
operator $\mathcal{O}^{'L}_{ub,d}$ or $\mathcal{O}^{'L}_{ub,s}$, and the superscript ($L$) will be omitted from now on. Strange number conversed or violated processes are induced by corresponding operators, which is summarized as,
\begin{equation}
    \begin{aligned}
        \Lambda_b^0 \to \pi^0 \bar{\psi} \quad \text{and} \quad \Xi_b^- \to K^- \bar{\psi}, \qquad \text{induced by $\mathcal{O}^{'L}_{ub,d}$}, \\
         \Lambda_b^0 \to K^0 \bar{\psi} \quad \text{and} \quad \Xi_b^- \to \pi^- \bar{\psi}, \qquad \text{induced by $\mathcal{O}^{'L}_{ub,s}$}. \\
    \end{aligned}
    \label{operators}
\end{equation}

In the framework of QCD factorization approach, the longitudinal momentum of the quarks in the energetic final state meson is at the scale of $m_b$ and the exchanged gluon have virtuality of order $m_b\Lambda_{\text{QCD}}$, which can be treated perturbatively.
Then we calculate the hard-scattering contributions, such as the ones shown in Fig.~\ref{fig:hadron-final-states}.
%
The decay amplitudes are written as
%
\begin{equation}{\label{Eq:amplitudes`with`spinor}}
      i \mathcal{M} = \eta_{\Delta s}
C^{L,R}_{u_ad_b,d_c} \zeta^{\mathcal{B} \to P}
\bigg(
\bar{v}_{\psi}^{\mathcal{C}}(q) 
    P_{R}\frac{\slashed{n}}{2}\,
    u_{\mathcal{B}}(p{'}) \bigg),
\end{equation}
where the sign factor $\eta_{\Delta s}=-1$ for strange flavor conserved processes $\Lambda_b^0\to\pi^0$ and $\Xi_b^-\to K^-$, while $\eta_{\Delta s}=+1$ for strange flavor violated processes $\Lambda_b^0\to K^0$ and $\Xi_b^-\to \pi^-$. The convention for the sign factor arises from the inconsistency between the quark flavor order in the operator $\mathcal{O}$ and the definition of the light-cone distribution amplitudes.

The factorization formula of the form factor $\zeta^{\mathcal{B} \to P}$ is given by
%
\begin{equation}{\label{eq:from`factor`analytical}}
\begin{aligned}
\zeta^{\mathcal{B} \to P} & =f_{P}f_{\mathcal{B}}^{(2)}
\int_{0}^{\infty}d\omega\,\omega\int_{0}^{1}du\int_{0}^{1}dx
\mathcal{J}^{\mathcal{B} \to P }(x,u,\omega,\mu)
\phi_{P}(x)
\psi_{2}(u,\omega),
\end{aligned}
\end{equation}
%H(x,u,\omega,\mu)$H(x,u,\omega,\mu)$ is the hard function with $H(x,u,\omega,\mu)=1$ at the tree level
where $f_{P(\mathcal{B})}$ is the decay constant of particle $P(\mathcal{B})$, $\mathcal{J}^{\mathcal{B} \to P }(x,u,\omega,\mu)$ is the corresponding hard-scattering kernel and $\phi_P(x)$ and $\psi_2(u,\omega)$ are the leading twist light-cone distribution amplitudes of the $P$ meson and $\mathcal{B}$ baryon \cite{Ball:2008fw,Bell:2013tfa,Beneke:2000ry,Grossman:2015cak},
%
\begin{equation}
    \left\langle P(p)|\,[\bar{q}(t\bar{n})]_{A}\,[t\bar{n},0]\,[q(0)]_{B}\,|0\right\rangle =\dfrac{if_{P}}{4}\,\bar{n}\cdot p\,\bigg[\,\dfrac{\slashed{n}}{2}\,\gamma_{5}\,\bigg]_{BA}\int_{0}^{1}dx\,e^{ixt\bar{n}\cdot p}\,\phi_{P}(x,\mu),
    \label{pi LCDA}
\end{equation}
with the momentum fraction $x$ of anti-quark $\bar{q}$ in the meson $P$, and
\begin{equation}
\begin{aligned} 
\bra{0}[u_{i}(t_{1}\bar{n})]_{A}&\,[0,t_{1}\bar{n}]\,[d_{j}(t_{2}\bar{n})]_{B}\,[0,t_{2}\bar{n}]\,[b_{k}(0)]_{C}\ket{\Lambda_{b}^0(p{'})}
\\
= &\dfrac{1}{6} \dfrac{\epsilon^{ijk}}{4}\,f_{\Lambda_{b}}^{(2)}(\mu)\,[u_{\Lambda_{b}}(p{'})]_{C}\,\bigg[\,\dfrac{\slashed{\bar{n}}}{2}\,\gamma_{5}\,C^{T}\,\bigg]_{BA}\int_{0}^{\infty}d\omega\,\omega\int_{0}^{1}du\,e^{-i\omega(t_{1}u+it_{2}\bar{u})}\,\psi_{2}(u,\omega),  
\\
 \bra{0}[d_{i}(t_{1}\bar{n})]_{A}&\,[0,t_{1}\bar{n}]\,[s_{j}(t_{2}\bar{n})]_{B}\,[0,t_{2}\bar{n}]\,[b_{k}(0)]_{C}\ket{\Xi_{b}^{-}(p{'})}
 \\
= & \dfrac{1}{6}\dfrac{\epsilon^{ijk}}{4}\,f_{\Xi_{b}}^{(2)}(\mu)\,[u_{\Xi_{b}^{-}}(p{'})]_{C}\,\bigg[\,\dfrac{\slashed{\bar{n}}}{2}\,\gamma_{5}\,C^{T}\,\bigg]_{BA}\int_{0}^{\infty}d\omega\,\omega\int_{0}^{1}du\,e^{-i\omega(t_{1}u+it_{2}\bar{u})}\,\psi_{2}(u,\omega),
\end{aligned}
\label{Baryon LCDA}
\end{equation}
%
where $\omega_i=(n\cdot k_i)$ represent the momentum components of the spectator quark respectively. We use the convention $\omega_1=u \omega$, $\omega_2=\bar{u} \omega$ with $\omega=\omega_1+\omega_2$, where $u$ and $\bar{u}$ represent the momentum fraction of the spectator quark in the light quark pair. 
The coupling constants $f_{\mathcal{B}}$ for $\Lambda_b^0$ and $\Xi_b^-$, in the
heavy-quark limit, are defined by \cite{Bell:2013tfa}, respectively,
%
\begin{equation}{\label{Eq:definition-decay-constants}}
\begin{aligned}
    \epsilon_{ijk} \langle 0| u^{iT}_{\alpha}(0) d^{j}_{\beta}(0) b^{k}_{\gamma}(0) |\Lambda_b^0(p{'})\rangle &\equiv \frac{1}{4} \left\{ f_{\Lambda_b}^{(1)} [\gamma_5 C^{T}]_{\beta\alpha} + f_{\Lambda_b}^{(2)} [\slashed{v}\gamma_5 C^{T}]_{\beta\alpha}\right\} \left[u_{\Lambda_b}(p{'})\right]_{\gamma}\\
    %
    \epsilon_{ijk} \langle 0| d^{iT}_{\alpha}(0) s^{j}_{\beta}(0) b^{k}_{\gamma}(0) |\Xi_b^-(p{'})\rangle &\equiv \frac{1}{4} \left\{ f_{\Xi_b}^{(1)} [\gamma_5 C^{T}]_{\beta\alpha} + f_{\Xi_b}^{(2)} [\slashed{v}\gamma_5 C^{T}]_{\beta\alpha}\right\} \left[u_{\Xi_b}(p{'})\right]_{\gamma}.
\end{aligned}
\end{equation}

%
%where $u$ and $\bar{u}$ represent the momentum fraction of light quarks in baryons, and $\omega$ is the sum of the two light quarks $n$-direction momenta.
%
The gauge links in Eq.~(\ref{Baryon LCDA}) is used to preserve the gauge invariance,
%
\begin{equation}
[t\bar{n},0]=\mathrm{P}\,\mathrm{exp}\bigg[\,ig\int_{0}^{t}dx\,\bar{n}\cdot A(x\bar{n})\,\bigg] ,
\end{equation}
%
which do not affect our calculations at the leading order of QCD.
The leading-twist LCDAs of pseudoscalar mesons can be expanded using
Gegenbauer polynomials \cite{Braun:2003rp},
%
\begin{equation}
\phi_{P}(x,\mu)=6x(1-x)\bigg[\,1+\sum_{n=1}^{\infty}a_{n}^{P}(\mu)\,C_{n}^{(3/2)}(2x-1)\,\bigg],
\end{equation}
%
and the leading-twist wave function
for the $\Lambda_{b}^0$ baryon is given by,
\begin{equation}
\psi_{2}(u,\omega)=u\,(1-u)\,\omega^{2}\,\dfrac{1}{\omega_{0}^{4}}\,e^{-\omega/\omega_{0}}.
\end{equation}
%
%where $\phi(x)$ and $\psi_2(u,\omega)$ represent the meson and baryon wave functions respectively.
In the limit of the SU(3) flavor symmetry, the wave function of $\Xi_b^-$ is  the same as that of $\Lambda_b^0$. 
TABLE \ref{tab:Input_Para} summarizes the numerical input parameters.
\begin{table} 	
\caption{The input parameters with renormalization scale $\mu_{0}=1\,\mathrm{GeV}$.} 	
\begin{spacing}{1.8} 		
\noindent \centering{}% 		
\begin{tabular}{ll|ll} 			
\hline 			
\hline  			
$\quad m_{\Lambda_{b}}=5.6196\,\mathrm{GeV}$ & \cite{ParticleDataGroup:2022pth}	& $\quad\tau_{\Lambda_{b}}=1.471\,\mathrm{ps}$ & \cite{ParticleDataGroup:2022pth} \\ 
$\quad m_{\Xi_{b}}=5.7970\,\mathrm{GeV}$ & \cite{ParticleDataGroup:2022pth}	& $\quad\tau_{\Xi_{b}}=1.572\,\mathrm{ps}$ & \cite{ParticleDataGroup:2022pth} \\			%
$\quad\omega_{0}=0.280\,_{-0.038}^{+0.047}\,\mathrm{GeV}$ & \cite{Wang:2015ndk} $\quad$ & 	$\quad f_{\Lambda_{b}}^{(2)}(\mu_{0})=0.030\pm 0.005\,\mathrm{GeV}^{3}$ \quad & \cite{Wang:2015ndk}$\quad$\\ 			
$\quad f_{\pi}=0.1304\pm0.0002\,\mathrm{GeV}$ \quad& \cite{Grossman:2015cak} $\quad$&	$\quad f_{K}=0.1562\pm0.0007\,\mathrm{GeV}$ & \cite{Grossman:2015cak} \\ 		
$\quad a_{1}^{\pi}(\mu_{0})=0$ & \cite{Grossman:2015cak} &	$\quad a_{2}^{\pi}(\mu_{0})=0.29\pm0.08$ & \cite{Grossman:2015cak}\\ 
$\quad a_{1}^{K}(\mu_{0})=-0.07\pm0.04$ & \cite{Grossman:2015cak} $\quad$ &	$\quad a_{2}^{K}(\mu_{0})=0.24\pm0.08$ & \cite{Grossman:2015cak}\\ 
%	
\hline  			
\hline 		
\end{tabular} 	
\end{spacing} 
\label{tab:Input_Para}
\end{table}
%

The corresponding hard-scattering functions are calculated as follows,
\begin{equation}
\begin{aligned}
    \mathcal{J}^{\Lambda_{b}^0\to\pi^{0}}(x,u,\omega,\mu)&=\frac{1}{\sqrt{2}}\big(\mathcal{J}_u(x,u,\omega,\mu)+\mathcal{J}_{\bar{u}}(x,u,\omega,\mu)\big),\\
    \mathcal{J}^{\Lambda_{b}^0\to K^{0}}(x,u,\omega,\mu)&=\mathcal{J}^{\Xi_{b}^{-}\to K^{-}}(x,u,\omega,\mu)=\mathcal{J}_{\bar{u}}(x,u,\omega,\mu),\\
    \mathcal{J}^{\Xi_{b}^{-}\to\pi^{-}}(x,u,\omega,\mu)&=\mathcal{J}_u(x,u,\omega,\mu),
\end{aligned}
\end{equation}
with
\begin{equation}
    \mathcal{J}_u(x,u,\omega,\mu)=\frac{1}{9}\frac{\pi\alpha_s(\mu)}{u \omega^2 x},\qquad
    \mathcal{J}_{\bar{u}}(x,u,\omega,\mu)=\frac{1}{9}\frac{\pi\alpha_s(\mu)}{\bar{u} \omega^2 x} ,
\end{equation}
where the $\frac{1}{\sqrt{2}}$ is isospin factor comes from $|\pi^0\rangle = \frac{1}{\sqrt{2}}(|u\bar{u}\,\rangle-|d\bar{d}\,\rangle)$.
Noted that the  asymptotic behaviors of the leading twist light-cone distribution amplitudes in the endpoint region are
\begin{equation}
    \phi_P(x)\sim x(1-x)\qquad  \psi_2(u,\omega)\sim u(1-u)\omega^2,
\end{equation}
which will cancel the divergent behavior in hard-scattering function $\mathcal{J}_u(x,u,\omega,\mu)$ and $\mathcal{J}_{\bar{u}}(x,u,\omega,\mu)$. Then the convolution integral in Eq.~\eqref{eq:from`factor`analytical} converges as noticed already in \cite{Li:2024htn,Wang:2011uv}.
%
Next, we  use the QCD
coupling constants as $\alpha_{s}(\small{2~ \mathrm{GeV}})\approx 0.3$ and other inputs summarized in TABLE.~\ref{tab:Input_Para}. The numerical
results for the form factors are
%
\begin{equation}
\begin{aligned}\label{equ:FormFactorMeson}
\zeta^{\Lambda_{b}^0\to\pi^{0}} & =(1.43\,_{-0.54}^{+0.46})\times10^{-2}\,[\mathrm{GeV}^2],\\
\zeta^{\Lambda_{b}^0\to K^{0}} & =(1.33\,_{-0.47}^{+0.40})\times10^{-2}\,[\mathrm{GeV}^2], \\
\zeta^{\Xi_{b}^{-}\to K^{-}} & =(1.33\,_{-0.47}^{+0.40})\times10^{-2}\,[\mathrm{GeV}^2],\\
\zeta^{\Xi_{b}^{-}\to\pi^{-}} & =(1.01\,_{-0.38}^{+0.33})\times10^{-2}\,[\mathrm{GeV}^2].
\end{aligned}
\end{equation}
%
Note that the mass dimension of form factor is $[\zeta]=2$, since the dimension of the baryon coupling constant $[f_{\mathcal{B}}]=3$.

Keep in mind that we take the heavy quark limit during the calculation for heavy baryon to light meson transition form factors, and the reliability of our results is best when the momentum transfer $q^2=0$. 
To extrapolate form factors $\zeta(q^2=0)$ toward $\zeta(q^2=m_{\psi}^2)$, we introduce the simplest single-pole model to describe the $q^2$ dependence of form factor $\zeta(q^2)$ \cite{Wirbel:1985ji,Shi:2024uqs},
\begin{equation}
\label{sig pol}
    \zeta(q^2)=\frac{1}{1-q^2/m^2_{\text{pole}}}\zeta(q^2=0).
\end{equation}
Here the denominator is introduced to describe the threshold Behaviour below the onset of the continuum. 
Frankly, the form factor has a pole at the mass of the lowest state that related to the operators in Eq.~\eqref{operators}. 
For instance, $m_{\rm pole}$ is the mass of $\Lambda_b^0(\frac{1}{2}^+)$ for $\Lambda_{b}^0\to\pi^{0} \,/\Xi^-_{b}\to K^{-}$ transition, as $\Lambda_b^0(\frac{1}{2}^+)$ is the lowest state of operator $\mathcal{O}^{'L}_{ub,d}$, while $m_{\rm pole}$ is the mass of $\Xi_b^0(\frac{1}{2}^+)$ for $\Lambda_{b}^0\to K^{0}\,/\Xi^-_{b}\to \pi^{-}$ transition.

The branching fractions of $\mathcal{B} \to P \bar{\psi}$ are expressed as  
\begin{equation}
\label{equ:BRmeson}
\mathcal{BR}(\mathcal{B} \to P \bar{\psi})
=\frac{|\Vec{q}_{\psi}|}{4 \pi \Gamma_{\mathcal{B}}  }\left|C^{L}_{u_ad_b,d_c}\right|^2     \left|\zeta^{\mathcal{B}\to P}(q^2)\right|^2,
\end{equation}
%\begin{equation}
%\begin{aligned}\label{equ:BRmeson}
%\mathcal{BR}(\Lambda_b \to \pi^0 \bar{\psi})&= \frac{|\Vec{q}_{\psi}|}{4 \pi \Gamma_{\Lambda_b}}  \ \left|C^{L}_{ub,d}\right|^2 
%     \left|\zeta^{\Lambda_{b} \to \pi^0}(q^2)\right|^2,\\
%     \mathcal{BR}(\Lambda_b \to K^0 \bar{\psi})&= \frac{|\Vec{q}_{\psi}|}{4 \pi \Gamma_{\Lambda_b}}  \ \left|C^{L}_{ub,s} \right|^2 
%     \left|\zeta^{\Lambda_{b} \to K}(q^2)\right|^2, \\
%        \mathcal{BR}(\Xi_b \to K^- \bar{\psi})&= \frac{|\Vec{q}_{\psi}|}{4 \pi \Gamma_{\Xi_b}}  \ \left|C^{L}_{ub,d} \right|^2 
%     \left|\zeta^{\Xi_{b} \to K^-}(q^2)\right|^2, \\  
%             \mathcal{BR}(\Xi_b \to \pi^- \bar{\psi})&= \frac{|\Vec{q}_{\psi}|}{4 \pi \Gamma_{\Xi_b}}  \ \left|C^{L}_{ub,s} \right|^2 
%     \left|\zeta^{\Xi_{b} \to \pi^-}(q^2)\right|^2.
%\end{aligned}
%\end{equation}
where $(u_ad_b,d_c)$ represents $(ub,d)$ or $(ub,s)$ for effective operators $ \mathcal{O}^{L}_{ub,d}$ or $ \mathcal{O}^{L}_{ub,s}$, $|\Vec{q}_{\psi}|$ is the momentum of the dark baryon $\bar{\psi}$ 
\begin{equation}
   |\Vec{q}_{\psi}|= \frac{\sqrt{(m_{\mathcal{B}}^2 - (m_{\psi}+m_P)^2)(m_{\mathcal{B}}^2 - (m_{\psi}-m_P)^2)}}{2 m_{\mathcal{B}}},
\end{equation}
and $\Gamma_{\mathcal{B}}$ ($m_{\mathcal{B}}$) is the decay width (mass) of the baryon $\mathcal{B}$.




==> 3-3-Calculation-radiative.tex <==
\subsection{Radiative semi-invisible decay of $\Lambda_b^0\to \gamma \bar\psi$}
%
\begin{figure}
\begin{centering}
\includegraphics[width=0.45\textwidth]{Fig/gamma-final-states1-Li.eps}
\par\end{centering}
\caption{The Feynman diagram for $\Lambda_b^0 \to \gamma\bar{\psi}$ with the bold line representing the $b$ quark.}
\label{FIG:Lambda_b_to_gamma_psi}
\end{figure}
%
For the radiative decay processes $\Lambda_b^0 \to \gamma \bar{\psi}$ showed in FIG. \ref{FIG:Lambda_b_to_gamma_psi},
the decay amplitudes can be expressed as,
%
\begin{equation}{\label{Eq:baryon-gamma-amplitude}}
     i \mathcal{M} =
C^{L,R}_{u_ad_b,d_c}
\bigg(
\bar{v}_{\psi}^{\mathcal{C}}(q)
    \langle \gamma(p)|
    \mathcal{O}^{'L,R}_{u_ad_b,d_c} |\Lambda_{b}^0(p')\rangle \bigg).
\end{equation}
%
%there are hadronic matrix elements need to be deal with.
The transition amplitudes associated with the right-handed operators $\mathcal{O}_{ub,d}^{'R} $ and $ \mathcal{O}_{ud,b}^{'R}$ always vanish for the same reason we have mentioned previously in the hadronic semi-invisible decays.  
The hadronic matrix elements in Eq. (\ref{Eq:baryon-gamma-amplitude}) could be parameterized in terms of two form factors,
%
\begin{equation}
    \langle \gamma(p)|
    \mathcal{O}^{'L}_{u_ad_b,d_c} |\Lambda_{b}^0(p')\rangle 
    = \bigg( 
    \zeta^{\Lambda_b \to \gamma}_1 \frac{\slashed{p}}{m_{\Lambda_{b}}^2} i\sigma^{\mu\nu} P_R + \zeta^{\Lambda_b \to \gamma}_2 \frac{\slashed{q}}{m_{\Lambda_{b}}^2} i\sigma^{\mu\nu} P_L 
    \bigg) u_{\Lambda_b}(p')\epsilon^{*}_{\mu}p_{\nu}.
\end{equation}
%
In the heavy quark limit, $\zeta^{\Lambda_b \to \gamma}_{2}$ is negligible due to the equation of motion of $\bar\psi$, similarly to the case of hadronic semi-invisible decays in the previous subsection. 
Additionally, only the diagram involving the coupling of the photon to the $d$ quark contributes to the final result. 
The photon radiation from $b$ quark is suppressed by $m_b$ in heavy quark propagator.
The contribution of the radiation from $u$ quark is also neglected,  
which is proportional to $\slashed{q}$ rather than $\slashed{p}'$, thus is irrelevant to the form factor $\zeta_1$.

In the heavy quark limit, the transition amplitude for operator $\mathcal{O}^{'L}_{ud,b}$ vanishes in our calculation. We can also arrive at this conclusion by considering the amplitude at the partonic level, which can be factorized as a product of two transition matrix elements in the spin space, $i\mathcal{M}\propto  \langle\bar{\psi}(q)|\,\bar{\psi}^{\mathcal{C}} b_R \, | b(m_bv)\rangle\,
 \langle \gamma(p)| \,  \bar{u}^{\mathcal{C}}_L d_L \,|u(k_1) d(k_2)\rangle$.
The second matrix element describes the transition of a quark pair to the photon, with the initial momentum $k$,  the transfer momentum $r$ and the final state momentum $p$. Its amplitude is proportional to the polarization vector $\epsilon_{\mu}$ of the photon. Considering momentum conservation $k+r=p$ and on-shell condition $p^2=0$, there are two independent Lorentz-invariant amplitudes proportional to $p\cdot \epsilon$ and $r\cdot \epsilon$ respectively.
In the heavy quark limit, we neglect the momentum $k\sim$ $\Lambda_{\text{QCD}}$ of the spectator quarks. Therefore, the second transition matrix element must be proportional to $p \cdot \epsilon=r\cdot \epsilon$, which is zero after implementing the Ward Identity $p\cdot\epsilon=0$. 

The non-vanishing amplitude $\Lambda_b^0\to\gamma \bar{\psi}$ defined by $\mathcal{O}_{ub,d}^{'L}$ is given by,
%
\begin{equation}
\begin{aligned}
i\mathcal{M}&=
C^{L}_{ub,d} \zeta^{\Lambda_{b}^0\to\gamma} \bigg(\bar{v}_{\psi}^{\mathcal{C}}(q)
P_{R}
\dfrac{\slashed{n}}{2}
\slashed{\epsilon}
\dfrac{\slashed{\bar{n}}}{2} u_{\Lambda_{b}}(p{'}) \bigg).
\end{aligned}
\end{equation}
%
  The form factors can be factorized as
\begin{equation}
\begin{aligned}
\zeta^{\Lambda_{b}^0\to\gamma}
=f_{\Lambda_{b}}^{(2)}\int_{0}^{\infty}d\omega\,\omega\int_{0}^{1}du\mathcal{J}^{\Lambda_{b}^0\to\gamma}(u,\omega,\mu)\psi_{2}(u,\omega),
\end{aligned}
\end{equation}
%
where $\mathcal{J}^{\Lambda_{b}^0\to\gamma}(u,\omega,\mu)$ is the hard-scattering kernel for $\Lambda_b \to \gamma$ transition,
\begin{equation}
\begin{aligned}
\mathcal{J}^{\Lambda_{b}^0\to\gamma}(u,\omega,\mu) &=\dfrac{1}{4}\bigg(\dfrac{Q_{d}(\mu)}{\bar{u}\omega}\bigg),
\end{aligned}
\end{equation}
where the electric charge of the light quark $d$ is $Q_{d}(\mu)=-\frac{1}{3}e(\mu)$. 
%
%
The numerical result for the form factor of the spectator processes
$\Lambda_{b}^0\to\gamma\bar{\psi}$ is,
%
\begin{equation}
\begin{aligned}\label{equ:FormFactorGamma}
 \zeta^{\Lambda_{b}^0\to\gamma}=(2.74\,_{-0.65}^{+0.59}) \times 10^{-3}\,[\mathrm{GeV^2}] ,
\end{aligned}
\end{equation}
%
%
whose input is shown in TABLE \ref{tab:Input_Para} with $\alpha_{em}(2~ \mathrm{GeV})\approx 1/133$ \cite{Erler:1998sy}. 
The single-pole model is also used to describe the $q^2$ dependence of form factor $\zeta(q^2)$,
\begin{equation}
\label{sig pol2}
    \zeta(q^2)=\frac{1}{1-q^2/m^2_{\Lambda_b}}\zeta(q^2=0),
\end{equation}
where $m_{\Lambda_b}$ is the mass of $\Lambda_b^0(\frac{1}{2}^+)$.
Then the branching ratio 
for $\Lambda_{b}^0\to\gamma\bar{\psi}$ with the operator $\mathcal{O}_{ub,d}^{'L}$ is  estimated as
\begin{equation}
\begin{aligned}\label{equ:BRgamma}
       \mathcal{BR} ({\Lambda_b^0\to\gamma\bar{\psi}})
  %  &= \frac{|\Vec{q}_{\psi}|}{8 \pi m_{\Lambda_b}^2 \Gamma_{\Lambda_b}} 
   % \bigg( \frac{1}{2} \sum_{spin} \sum_{spin} |i \mathcal{M}|^2 \bigg) 
    &= 
    \frac{|\Vec{q}_{\psi}|}{8 \pi \Gamma_{\Lambda_b}}  \ |C^{L}_{ub,d}|^2
\left|\zeta^{\Lambda_{b}^0\to\gamma}(q^2=m_{\psi}^2)\right|^2.
\end{aligned}
\end{equation}

==> 3-QCDSR_for_decay_constant.tex <==
\section{The coupling constants of baryons in QCD sum rules}{\label{Appen-QCD-input}}
Here we derive the QCD sum rules for the coupling constants $\lambda_{\Lambda_b}^{L,R}$, $\lambda_{\Xi_c}^{L,R}$ and ${\lambda_{\Lambda}^{L,R}}$. For the heavy baryons $\Lambda_b^0$ and $\Xi_c^0$
, its definition of coupling constants $\lambda_{\mathcal{B}}$ in the heavy-quark limit could be written as \cite{Grozin:1992td, Groote:1997yr, Ball:2008fw, Ali:2012pn, Bell:2013tfa}, 
\begin{equation}\label{matrix-elements}
      \bra{0} \mathcal{J}_{\mathcal{B}}^{(1,2)}(0) \ket{\mathcal{B}\left(p\right)}\equiv\lambda_{\mathcal{B}}^{(1,2)} \ u_{\mathcal{B}}\left(p\right),
\end{equation}
where the current $\mathcal{J}_{\mathcal{B}}$ for $\Lambda_b^0$ and $\Xi_c^0$ are respectively shown as,
\begin{equation}{\label{currents}}
    \begin{aligned}
    \mathcal{J}_{\Lambda_{b}}^{(1)}(x) &= \epsilon_{ijk} \left[  u^{iT}(x) \mathcal{C} \gamma_5 d^j(x) \right]  b^k(x),\ \mathcal{J}_{\Lambda_{b}}^{(2)}(x) = \epsilon_{ijk} \left[  u^{iT}(x) \mathcal{C} \gamma_5 \slashed{v} d^j(x) \right]  b^k(x),\\
    \mathcal{J}_{\Xi_{c}}^{(1)}(x) &= \epsilon_{ijk} \left[  d^{iT}(x) \mathcal{C} \gamma_5 s^j(x) \right]  c^k(x),\ \mathcal{J}_{\Xi_{c}}^{(2)}(x) = \epsilon_{ijk} \left[  d^{iT}(x) \mathcal{C} \gamma_5 \slashed{v} s^j(x) \right]  c^k(x).
    \end{aligned}
\end{equation}
whose form is determined by $P$ parity and the heavy quark symmetry, besides, the $\mathcal{C}$ is the charge conjugation matrix and $v^{\mu}$ is the four-speed of heavy quark. They are the largest coupling to the $\Lambda_b^0$ and $\Xi_c^0$, respectively. The above definitions can be cast into a Lorentz-invariant form by defining the
most general matrix elements as \cite{Bell:2013tfa},
\begin{equation}
    \epsilon_{ijk} \bra{0} u^{iT}_{\alpha}(0) d^{j}_{\beta}(0) b^{k}_{\gamma}(0) \ket{\Lambda_b^0} \equiv \frac{1}{4} \left\{ \lambda_{\Lambda_b}^{(1)} [\gamma_5 \mathcal{C}^{T}]_{\beta\alpha} + \lambda_{\Lambda_b}^{(2)} [\slashed{v}\gamma_5 \mathcal{C}^{T}]_{\beta\alpha}\right\} \left[u_{\Lambda_b}\left(p\right)\right]_{\gamma}
\end{equation}
for the $\Lambda_b^0$ baryon and 
\begin{equation}
    \epsilon_{ijk} \bra{0} d^{iT}_{\alpha}(0) s^{j}_{\beta}(0) c^{k}_{\gamma}(0) \ket{\Xi_c^0} \equiv \frac{1}{4} \left\{ \lambda_{\Xi_c}^{(1)} [\gamma_5 \mathcal{C}^{T}]_{\beta\alpha} + \lambda_{\Xi_c}^{(2)} [\slashed{v}\gamma_5 \mathcal{C}^{T}]_{\beta\alpha}\right\} \left[u_{\Xi_c}\left(p\right)\right]_{\gamma}
\end{equation}
for the $\Xi_c$ baryon.
We find the relation between our factor $\lambda_{\mathcal{B}}^{L,R}$ and standard baryon coupling constants $\lambda_{\mathcal{B}}^{(1,2)}$ satisfy that are shown in TABLE \ref{tab:relation_coupling_constants}. Fortunately, for the numerical value of the couplings, in Ref. \cite{Groote:1997yr} have the result：$\lambda_{\Lambda_b}^{(1)}\approx\lambda_{\Lambda_b}^{(2)}$. Besides, $\Lambda_b^0$ and $\Xi_c^0$ have the same construction of the currents in Eq.\eqref{currents}, then, we quote the results: $\lambda_{\mathcal{B}}^{(1)} \approx \lambda_{\mathcal{B}}^{(2)}$.
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
      $(u_ad_b,d_c)$   & \quad   $(ud,b)$ \quad &    \quad $(ub,d)$ \quad &   \quad $(cd,s)$ \quad &  \quad   $(cs,d)$ \quad \tabularnewline
\hline 
\hline 
       $\lambda_{\mathcal{B}}^L$  & $-\frac{1}{2} \lambda_{\Lambda_b}^{(1)}$ & $-\frac{1}{4} \lambda_{\Lambda_b}^{(2)}$ & \quad $\frac{1}{4} \lambda_{\Xi_c}^{(2)}$& $-\frac{1}{4} \lambda_{\Xi_c}^{(2)}$  \\
\hline 
       $\lambda_{\mathcal{B}}^R$  & $\quad \frac{1}{2} \lambda_{\Lambda_b}^{(1)}$  & $ \quad \frac{1}{4} \lambda_{\Lambda_b}^{(1)}$& $-\frac{1}{4}\lambda_{\Xi_c}^{(1)}$& \quad $\frac{1}{4}\lambda_{\Xi_c}^{(1)}$ \\
       \hline
    \end{tabular}
    \caption{The relation between the coupling $\lambda_{\mathcal{B}}^{L,R}$ in \eqref{our_coupling} and standard baryon coupling constants $\lambda_{\mathcal{B}}^{(1,2)}$ in \eqref{matrix-elements}.}
    \label{tab:relation_coupling_constants}
\end{table}
% \begin{equation}
%   \lambda_{\mathcal{B}}^{L}=-\frac{1}{2}\lambda_{\mathcal{B}}, \quad \lambda_{\mathcal{B}}^{R}=\frac{1}{2}\lambda_{\mathcal{B}}.
% \end{equation}
%where $u_{\Lambda_b}(p)$ is the spinor representation of $\Lambda_b$ baryon and the current $\mathcal{J}_{\Lambda_b}$ defines as
%\begin{equation}{\label{currents}}
%    \begin{aligned}
 %   \mathcal{J}_{\Lambda_{b}}(x) &= \epsilon^{ijk} \left[  u_i^T(x) C \gamma_5 d_j(x) \right] P_R b_k(x).
 %   \end{aligned}
%\end{equation}
%Since the decay constants $\lambda_{\Lambda_b}^{L,R}$ are non-perturbative quantities, we have to utilize several QCD methods, including QCD sum rules \cite{Shifman:1978bx,Shifman:1978by,Colangelo:2000dp}, lattice QCD \cite{Wilson:1974sk,PhysRevD.78.054505} and Dyson-Schwinger equation \cite{Luecker:2009bs}, to approximately estimate their value. 
% The coupling constants $\lambda_{\Lambda_b}$ and $\lambda_{\Xi_c}$ have been studied with the QCD sum rules approach in Ref. \cite{Groote:1997yr, Wang:2010fq, Ball:2008fw,Bagan:1992tp}. {\color{blue}{[connection: since there are other people's results, why we need to reproduce the coupling constants?] }}
To numerically determine the coupling constants $\lambda_{\mathcal{B}}^{L,R}$, we only need calculate the corresponding correlation functions,
\begin{equation}{\label{eq_correlator}}
       \begin{aligned}
             \Pi_{\mathcal{B}}(q) = i \int d^4 x e^{iq \cdot x} \bra{0}T\left\{  \mathcal{J}_{\mathcal{B}}^{(1)}(x) \bar{\mathcal{J}}_{\mathcal{B}}^{(1)}(0)  \right\}\ket{0},
       \end{aligned}
\end{equation}
following the usual way of the QCD sum rules.  The correlation function could be decomposed as: 
\begin{equation}{\label{eq_after_insert_cs}}
\begin{aligned}
     \Pi_{\mathcal{B}}(q)&
      &= \slashed{q}   \Pi_{\mathcal{B}, 0}(q^2) + \Pi_{\mathcal{B}, 1}(q^2).
\end{aligned}
\end{equation} 
Then we use dispersion relations and take Borel transformations for both hadronic part and partonic part following the standard steps of QCD sum rules \cite{Shifman:1978bx,Shifman:1978by,Colangelo:2000dp}. The final results are obtained as follows,
\begin{equation}{\label{eq:final-result}}
     \begin{aligned}
                    \left(\lambda_{\mathcal{B}}  \right)^2 & e^{-m_{\mathcal{B}}^2/M^2} = \frac{1}{\pi}\int_{m_{b,c}^2}^{s_0^{\mathcal{B}}}   ds\ e^{-s/M^2}\ \mathbf{Im}~\!\Pi_{\mathcal{B}, 0}  \left(s \right)_{\textbf{OPE}}. 
     \end{aligned}
\end{equation}
 When evaluating the correlation function Eq.\eqref{eq_correlator} at leading order of $\alpha_s$ and the vaccum condensates up to dimension $d=6$, the corresponding diagrams are illustrated in FIG.\ref{Fig:Baryon_correlator-total}.
\input{Feynman-diagram/total_per_and_non-per}Their analytical results for Eq. \eqref{eq:final-result} are given by,
\begin{equation}{\label{eq:OPE_result}}
                 \begin{aligned}
             % \mathcal{J}_{\Lambda_Q} &= \epsilon^{ijk} \left[  u_i^T C \gamma_5 d_j \right] P_R Q_k, \\
            \mathbf{Im}\Pi^{(pert)}_{\Lambda_Q, 0}(s) 
           &= \frac{m_Q^4}{2^{9}\pi^3} \left(   
           \frac{1}{x^2} - \frac{8}{x} +8x -  x^2
           -12ln(x)
           \right), \\
            \mathbf{Im} \Pi^{(\left< \bar{q}q \right>)}_{\Lambda_Q, 0} (s) 
          &=- 
          \frac{m_q \left<\bar{q}q\right>}{2^4\pi}   (1-x^2),
          \\
            \mathbf{Im} \Pi^{(\left< GG\right>)}_{\Lambda_Q, 0} (s)
         &=  \frac{\left<g^2_s G^2\right>}{3 \cdot 2^{10} \pi^3} (1 + 4x-5x^2),
          \\
         \Pi^{(\left<\bar{q} G q \right>)}_{\Lambda_Q, 0}(q^2) 
          &=  \frac{7 m_q\left< \bar{q}Gq \right>}{3 \cdot 2^5 \pi^2 (m_Q^2- q^2)}, \\
             \Pi^{(\left< \bar{q}q \right>^2)}_{\Lambda_Q, 0} (q^2)
                 &=
                \frac{{\left< \bar{q}q \right>^2}}{6(m_Q^2-q^2)},
                 \end{aligned} 
           \end{equation}
and 
\begin{equation}{\label{eq:OPE_result2}}
                 \begin{aligned}
             % \mathcal{J}_{\Xi_Q} &= \epsilon^{ijk} \left[  d_i^T C \gamma_5 s_j \right] P_R Q_k, \\
        \mathbf{Im}\Pi^{(pert)}_{\Xi_Q, 0}(s) 
           &= \frac{m_Q^4}{2^{9}\pi^3} \left(   
           \frac{1}{x^2} - \frac{8}{x} +8x -  x^2
           -12ln(x)
           \right), \\
            \mathbf{Im} \Pi^{(\left< \bar{q}q \right>)}_{\Xi_Q, 0} (s) 
          &= 
          \frac{m_s\left[\left<\bar{s}s\right> -  2\left<\bar{q}q\right> \right]}{2^5\pi}  (1-x^2),
          \\
            \mathbf{Im} \Pi^{(\left< GG\right>)}_{\Xi_Q, 0} (s)
         &=  \frac{\left<g^2_s G^2\right>}{3 \cdot 2^{10} \pi^3} (1 + 4x-5x^2),
          \\
         \Pi^{(\left<\bar{q} G q \right>)}_{\Xi_Q, 0}(q^2) 
          &=  \frac{ m_s \left[6\left< \bar{q}Gq \right> + \left< \bar{s}Gs \right>\right]}{3 \cdot 2^6 \pi^2 (m_Q^2- q^2)}, \\
             \Pi^{(\left< \bar{q}q \right>^2)}_{\Xi_Q, 0} (q^2)
                 &=
                \frac{{\left< \bar{q}q \right>\left< \bar{s}s \right>}}{6(m_Q^2-q^2)},
                 \end{aligned} 
           \end{equation}
where $x= \frac{m_Q^2}{s}$. 
The values of input parameters are shown as follow: 
$m_b = 4.60 \pm 0.10 \ \text{GeV}$, 
$m_c = 1.35 \pm 0.10 \ \text{GeV}$,
$m_s = 0.12  \pm 0.01\ \text{GeV}$, $m_{\Lambda_b}=5.619 \ \text{GeV}$,
$m_{\Xi_c}=2.490 \ \text{GeV}$,
$m_{\Lambda}=1.116 \ \text{GeV}$ \cite{ParticleDataGroup:2022pth,Hu_2018}, and the light quarks $u$ and $d$ are taken as massless.  
On the other hand, the vacuum condensates are given by:  
$\left<\bar{q}q\right> = -(0.24 \pm 0.01\ \text{GeV})^3$, $\left<\bar{s}s\right> = (0.8 \pm 0.1) \left<\bar{q}q\right> $, $\left<g_s^2 GG \right> = 0.88 \pm 0.25\ \text{GeV}^4$, $\left< \bar{q} G q \right> = \left< \bar{q}g_s \sigma G q \right> = m_0^2 \ \left<\bar{q}q\right>$,  $\left< \bar{s} G s \right> = \left< \bar{s}g_s \sigma G s \right> = m_0^2\ \left<\bar{s}s\right>$ and $m_0^2= 0.8 \pm 0.1\ \text{GeV}^2$
at the energy scale $\mu = 1\ \text{GeV}$  \cite{Hu_2018,Xin:2023usd}. Finally, when setting the effective threshold at $\sqrt{s_0^{\Lambda_b}}=(6.5\pm 0.1)$ GeV for $\Lambda_b^0$ and $\sqrt{s_0^{\Xi_c}}=(3.2\pm 0.1)$ GeV for $\Xi_c^0$, we find 
\begin{equation}
\begin{aligned}
\lambda_{\Lambda_b}^{(1)} &= 
\left( 3.40 \pm 0.20 \pm 0.60 \right) \times10^{-2} 
\ \left[\text{GeV}^3\right], \\
\lambda_{\Xi_c}^{(1)} &= \left( 2.90 \pm 0.20 \pm 0.30 \right) \times 10^{-2} \ \left[\text{GeV}^3 \right],
\end{aligned}
\end{equation}
which are consistent with the previous works \cite{Groote:1997yr, Wang:2010fq, Ball:2008fw,Bagan:1992tp}.
Where the first uncertainty originates from the effective threshold $s_0^{\Lambda_b(\Xi_c)}$
and Borel parameter $M^2$, the second one arises from the other QCD
input parameters.
The dependence of the coupling constants $\lambda_{\Lambda_b}$ and $\lambda_{\Xi_c}$ on the Borel parameter $M^2$ are illustrated in FIG.\ref{fig:coupling-constants} (a) and (b).  

To compared with the result of $\Lambda_b$ and $\Xi_c$, we also calculated the coupling constant and the invisible decay of $\Lambda$ within QCD sum rules. For the light baryon $\Lambda$, without the heavy quark symmetry, the corresponding coupling  constants $\lambda_{\Lambda}^{L,R}$ is defined as \cite{PhysRevD.105.115005},
\begin{equation}
 \begin{aligned}
     \epsilon_{ijk} \bra{0} 
  \left[u^{i T}(0)\, C P_{L, R}\, d_b^j(0) \right] d_{Rc}^k(0)
  \ket{\Lambda\left(p\right)}\equiv \lambda_{\Lambda}^{L,R} P_Ru_{\Lambda}\left(p\right), 
 \end{aligned}
\end{equation}
where $(ud_b, d_c) = (ud, s)$ or $(us, d)$. The relation for each of the flavor configurations
$(ud_b, d_c)$ in the operators $O^{'L,R}_{ud_b, d_c}$ are listed in Ref. \cite{PhysRevD.105.115005}. Therefore, we only calculate the $\lambda_{\Lambda}^{L,R}$ with the operator $O^{'L,R}_{ud, s}$ after following the standard steps of QCD sum rules. When taking into account the leading order of $\alpha_s $ and the condensates up to dimension $d=6$, the OPE results are given by 
\begin{equation}{\label{eq:OPE_result_Lambda}}
                \begin{aligned}
    \mathbf{Im}\Pi_{\Lambda, 0}^{L, R (pert)}(s) 
    &= \frac{m_s^4}{2^{10}\pi^3} \left(   
           \frac{1}{x^2} - \frac{8}{x} +8x -  x^2
           -12ln(x)
           \right) ,
\\
    \mathbf{Im} \Pi^{L, R \left< \bar{q}q \right>}_{\Lambda, 0}(s) 
    &=   \frac{m_s \left<\bar{s} s\right> }{ 2^6 \pi}, 
\\
    \mathbf{Im} \Pi^{L,R \left< GG\right>}_{\Lambda, 0} (s)
        &=  \frac{\left<g^2_s G^2\right>}{3 \cdot 2^{11} \pi^3} (1 + 4x-5x^2),
\\
  \Pi^{L,R \left< \bar{q}G q \right>}_{\Lambda, 0}(q^2) 
  &=  \frac{ m_s  \left<\bar{s}Gs\right>}{3 \cdot 2^6 \pi^2 q^2},  \\
  % \Pi^{L/R(\left< \bar{q}q \right>^2)}_{\Lambda, 0}(s)
   %    &= 
   %    \frac{ m_s m_q \left<\bar{s}s \right> \left< \bar{q}\bar{q}\right>}{ 24  s^2}
                \end{aligned}
         \end{equation}
where $x= \frac{m_s^2}{s}$ and the mass of light quarks are neglected. The dependence of coupling constant $|\lambda_{\Lambda}^{L,R}|$ with the operator $O^{'L,R}_{ud, s}$ on Borel parameters $M^2$ is illustrated in FIG.\ref{fig:coupling-constants} (c), which determine the value of coupling constants as
\begin{equation}
    \left|\lambda^{L,R}_{\Lambda}\right| = \left( 5.4 \pm 0.3\pm 0.1\right) \times 10^{-3}\ \left[\text{GeV}^3\right].
\end{equation}


% Following the similar procedures, we also estimate $\lambda_{\Xi_c}$ form the correlation function \eqref{eq_correlator}

% \begin{equation}{\label{eq:OPE_result2}}
%                  \begin{aligned}
%              % \mathcal{J}_{\Xi_Q} &= \epsilon^{ijk} \left[  d_i^T C \gamma_5 s_j \right] P_R Q_k, \\
%         \mathbf{Im}\Pi^{(pert)}_{\Xi_Q, 0}(s) 
%            &= \frac{m_Q^4}{2^{9}\pi^3} \left(   
%            \frac{1}{x^2} - \frac{8}{x} +8x -  x^2
%            -12ln(x)
%            \right), \\
%             \mathbf{Im} \Pi^{(\left< \bar{q}q \right>)}_{\Xi_Q, 0} (s) 
%           &= 
%           \frac{m_s\left[\left<\bar{s}s\right> -  2\left<\bar{q}q\right> \right]}{2^5\pi}  (1-x^2),
%           \\
%             \mathbf{Im} \Pi^{(\left< GG\right>)}_{\Xi_Q, 0} (s)
%          &=  \frac{\left<g^2_s G^2\right>}{3 \cdot 2^{10} \pi^3} (1 + 4x-5x^2),
%           \\
%          \Pi^{(\left<\bar{q} G q \right>)}_{\Xi_Q, 0}(s) 
%           &=  \frac{ m_s \left[6\left< \bar{q}Gq \right> + \left< \bar{s}Gs \right>\right]}{3 \cdot 2^6 \pi^2 (m_Q^2- s)} , \\
%              \Pi^{(\left< \bar{q}q \right>^2)}_{\Xi_Q, 0} (s)
%                  &=
%                 \frac{{\left< \bar{q}q \right>\left< \bar{s}s \right>}}{6(m_Q^2-s)},
%                  \end{aligned} 
%            \end{equation}
% where $x= \frac{m_Q^2}{s}$. And the final result is,
% \begin{equation}
%     \lambda_{\Xi_c} = \left( 2.9 \pm 0.2 \pm 0.3 \right) \times 10^{-2} \ \left[\text{GeV}^3 \right].
% \end{equation}
% The dependence of the coupling constant $\lambda_{\Lambda_b}$ on the Borel parameter $M^2$ is illustrated in FIG.\ref{fig:coupling-constants} (b). 


% To evaluate the $\Lambda$ invisible decay in QCD sum rules, we have to estimate the corresponding coupling constants of $\Lambda$ baryon. 
% When taking into account the leading order of $\alpha_s $ and the condensates up to dimension $d=6$, the OPE results are given by 
% \begin{equation}{\label{eq:OPE_result_Lambda}}
%                 \begin{aligned}
%     \mathbf{Im}\Pi_{\Lambda, 0}^{L, R (pert)}(s) 
%     &= \frac{m_s^4}{2^{10}\pi^3} \left(   
%            \frac{1}{x^2} - \frac{8}{x} +8x -  x^2
%            -12ln(x)
%            \right) ,
% \\
%     \mathbf{Im} \Pi^{L, R \left< \bar{q}q \right>}_{\Lambda, 0}(s) 
%     &=   \frac{m_s \left<\bar{s} s\right> }{ 2^6 \pi}, 
% \\
%     \mathbf{Im} \Pi^{L,R \left< GG\right>}_{\Lambda, 0} (s)
%         &=  \frac{\left<g^2_s G^2\right>}{3 \cdot 2^{11} \pi^3} (1 + 4x-5x^2),
% \\
%   \Pi^{L,R \left< \bar{q}G q \right>}_{\Lambda, 0}(s) 
%   &=  \frac{ m_s  \left<\bar{s}Gs\right>}{3 \cdot 2^6 \pi^2 s},  \\
%   % \Pi^{L/R(\left< \bar{q}q \right>^2)}_{\Lambda, 0}(s)
%    %    &= 
%    %    \frac{ m_s m_q \left<\bar{s}s \right> \left< \bar{q}\bar{q}\right>}{ 24  s^2}
%                 \end{aligned}
%          \end{equation}
% where $x= \frac{m_s^2}{s}$ and the mass of light quarks are neglected. When implementing the Borel transformation, the dependence of coupling constants on Borel parameters $M^2$ is illustrated in FIG.\ref{fig:coupling-constants} (c), which determine the value of coupling constants as
% \begin{equation}
%     |\lambda^{L,R}_{\Lambda}| = \left( 5.4 \pm 0.3\pm 0.1\right) \times 10^{-3}\ \left[\text{GeV}^3\right].
% \end{equation}
% With such coupling constants of $\Lambda$ baryon, the corresponding sensitivity on $|y_{\xi\phi}|$ are illustrated as the solid lines in FIG.\ref{fig:constraint-mchi} and FIG.\ref{fig:constraint-mtotal}.


\begin{figure}[htb]
    \centering
    \subfigure[\quad Coupling constant of $\Lambda_b^0$ baryon]{
        \includegraphics[width=0.45\textwidth]{Fig/decay-constant-Lambda-b1.eps}}\\
    \subfigure[\quad Coupling constant of $\Xi_c^0$ baryon]{\includegraphics[width=0.45\textwidth]{Fig/decay-constant-Xic.eps}} 
    \subfigure[\quad Coupling constant of $\Lambda$ baryon]{\includegraphics[width=0.47\textwidth]{Fig/decay-constant-Lambda1.eps}}
    \caption{The $M^2$-dependence of $\Lambda_b^0 \left(\Xi_c^0,  \Lambda \right)$ coupling constants in different effective threshold $s_0^{\Lambda_b \left(\Xi_c,  \Lambda \right)}$.}
    \label{fig:coupling-constants}
\end{figure}





















% \section{the decay constant under the QCD sum rules}
% \label{sec:QCD-for-decay-constant}


% Among these QCD methods, we suggest to utilize QCD sum rules \cite{Shifman:1978bx,Shifman:1978by,Colangelo:2000dp} to determine the values of decay constants $\lambda_{\Lambda_b}^{L,R}$, as this method has already demonstrated success in predicting various hadronic decay constants \cite{Khodjamirian:2020btr,Narison:2015nxh,Lucha:2016puq,Hu_2018}.
% To estimate the decay constants $\lambda_{\Lambda_b}^{L,R}$ within QCDSR, we initiate with the correlation function of $\Lambda_b$ baryon: 
% \begin{equation}{\label{eq_correlator}}
%        \begin{aligned}
%              \Pi^{L,R}_{\Lambda_b}(q) = i \int d^4 x e^{iq \cdot x} \bra{0}T\left\{  \mathcal{J}^{L,R}_{\Lambda_b}(x) \bar{\mathcal{J}}^{L,R}_{\Lambda_b}(0)  \right\}\ket{0}.
%        \end{aligned}
% \end{equation}
% When inserting a complete set of baryon spectra into the correlation function and applying the dispersion relation, the correlation function can be rewritten as:
% \begin{equation}{\label{eq_after_insert_cs}}
% \begin{aligned}
%      \Pi^{L,R}_{\Lambda_b}(q)&= \left(\slashed{q}  P_L \right) \left\{  
%       \frac{
%       \left(\lambda^{L,R}_{\Lambda_b} \right)^2
%       }
%       { m_{\Lambda_b}^2 - q^2}
%       + \int_{t_{min}}^{\infty}
%       ds\ \frac{\rho^{L,R}_{\Lambda_b} \left(s \right)}{s-q^2}  \right\} \\
%       &= \left(\slashed{q}  P_L \right) \Pi^{L,R}_{\Lambda_b, 0}(q^2),
% \end{aligned}
% \end{equation} 
% where we isolate the pole of $\Lambda_b$-baryon in the first term, while the contributions from excited and continuum states are incorporated into the integral of the spectral density $\rho(s)$.
% For simplicity, we redefine the invariant correlation function $\Pi^{L,R}_{\Lambda_b, 0}(q^2)$ in the second line to represent the dynamic contribution.
% To determine the values of the decay constants $\lambda_{\Lambda_b}^{L,R}$, we must further expand the invariant correlation function of $\Lambda_b$ under the operator product expansion (OPE) \cite{Wilson:1969zs},
%  \begin{equation}
%  \begin{aligned}{\label{eq_OPE}}
%      \Pi^{L,R}_{\Lambda_b,0}(q^2)_{OPE}
%      =  \Pi_{\Lambda_b, 0}^{L, R (pert)}
%     + \Pi_{\Lambda_b, 0}^{L, R \left<\bar{q} q \right>} 
%     +\Pi_{\Lambda_b, 0}^{L, R \left< GG \right>}+ \Pi_{\Lambda_b, 0}^{L, R \left<\bar{q} G q \right>}  + \Pi_{\Lambda_b, 0}^{L, R \left<\bar{q} q \bar{q} q \right>} + \cdots,
%  \end{aligned}
%  \end{equation}
% where the correlation functions on the right-hand side represent contributions stemming from perturbative calculations, quark condensate, gluon condensate, mixed condensate, four-quark condensate, and so on. 
% When matching between Eq.\eqref{eq_after_insert_cs} and Eq.\eqref{eq_OPE}, the invariant correlation function $\Pi_{\Lambda_b,0}^{L,R}(q^2)$ satisfies
% \begin{equation}{\label{eq:matching_bef_sub}}
%      \Pi_{\Lambda_b, 0}^{L,R} (q^2)_{OPE}=   \frac{
%       \left(\lambda^{L,R}_{\Lambda_b} \right)^2
%       }
%       {  m_{\Lambda_b}^2 - q^2}
%       + \frac{1}{\pi}\int_{s_0^{\Lambda_b}}^{\infty}
%       ds\  \frac{\mathbf{Im}~\! 
%       \Pi_{\Lambda_b, 0}^{L,R}  \left(s \right)_{OPE}}{s-q^2},
% \end{equation}
% where we assume a quark-hadron duality for the spectral density $\rho_{\Lambda_b}^{L,R}$ as
% \begin{equation}{\label{eq:quark-hadron-dual-assup}}
%     \int_{t_{min}}^{\infty}
%       ds\ \frac{\rho^{L,R}_{\Lambda_b} \left(s \right)}{s-q^2}  \simeq \frac{1}{\pi}\int_{s_0^{\Lambda_b}}^{\infty}
%       ds\  \frac{\mathbf{Im}~\! 
%       \Pi_{\Lambda_b, 0}^{L,R}  \left(s \right)_{OPE}}{s-q^2},
% \end{equation}
% with $s_0^{\Lambda_b}$ correspond to the effective threshold. 
% Taking into account the analytic continuation of $\Pi_{\Lambda_b, 0}^{L,R} (q^2)_{OPE}$ in Eq.\eqref{eq:matching_bef_sub}, 
% \begin{equation}
%     \Pi_{\Lambda_b, 0}^{L,R} (q^2)_{OPE} = \frac{1}{\pi}\int_{m_b^2}^{\infty}  ds\  \frac{\mathbf{Im}~\!  
%       \Pi_{\Lambda_b, 0}^{L,R}  \left(s \right)_{OPE}}{s-q^2},
% \end{equation}
% the decay constants $\lambda_{\Lambda_b}^{L,R}$ satisfy
% \begin{equation}\label{equ_dc_Im}
%     \frac{
%       \left(\lambda^{L,R}_{\Lambda_b} \right)^2
%       }
%       {  m_{\Lambda_b}^2 - q^2}
%       =
%       \frac{1}{\pi}\int_{m_b^2}^{s_0^{\Lambda_b}}
%       ds\  \frac{\mathbf{Im}~\! 
%       \Pi_{\Lambda_b, 0}^{L,R}  \left(s \right)_{OPE}}{s-q^2}.
% \end{equation}
% When evaluating the correlation function at leading order of $\alpha_s$ and the condensates up to dimension $d=6$, the corresponding diagrams are illustrated in FIG.\ref{Fig:Baryon_correlator-total}.
% \input{Feynman-diagram/total_per_and_non-per}
% If neglect the light quarks mass, the analytical results only depend on the contributions arose from the perturbative calculations and gluon condensates, given by
% \begin{equation}{\label{eq:OPE_result}}
%                  \begin{aligned}
%                               \mathbf{Im}\Pi_1^{L/R(pert)}(s) 
%            &= \frac{m_Q^4}{2^{10}\pi^3} \left(   
%            \frac{1}{x^2} - \frac{8}{x} +8x -  x^2
%            -12ln(x)
%            \right) \\
%             \mathbf{Im} \Pi^{L/R(\left< \bar{q}q \right>)}_1 (s) 
%           &= 
%           \frac{m_q \left< \bar{q}q\right>}{2^5 \pi }(1-x^2)
%           \\
%             \mathbf{Im} \Pi^{L/R(\left< GG\right>)}_1 (s)
%          &=  \frac{\left<g^2_s G^2\right>}{3 \cdot 2^{11} \pi^3} (1 + 4x-5x^2)
%           \\
%          \Pi^{L/R(\left<\bar{q} G q \right>)}_1(s) 
%           &=
%           - \frac{  m_q \left<\bar{q}Gq\right> }{ 2^{6}\pi^2 ( m_Q^2 - s)} \\
%              \Pi^{L/R(\left< \bar{q}q \right>^2)}_1 (s)
%                  &=
%                 \frac{ m_q^2 \left< \bar{q}q \right>^2   }{3 \cdot 2^{4} }   
%               \left[  \frac{3}{(m_Q^2 -s )^{2}}
%                + \frac{2 s}{(m_Q^2 -s )^{3}}
%               \right]
%                  \end{aligned} 
%            \end{equation}
% where $x= \frac{m_b^2}{s}$. 
% Obviously, since the correlation functions are independent of chirality, the decay constants with different chirality should be equal to each other, $|\lambda_{\Lambda_b}^{L}| = |\lambda_{\Lambda_b}^{R}|$.
% Note that the imaginary part of the correlation function in Eq.\eqref{eq:OPE_result} will diverge as $s\to\infty$,
% \begin{equation}
%     \mathop{lim}\limits_{s \to \infty} \mathbf{Im}~\! \Pi_{\Lambda_b, 0}^{L,R} (s)_{OPE} \sim s^2,
% \end{equation}
% which contradicts the convergence requirements of a dispersion relation. 
% Fortunately, the Borel transformation provides a feasible procedure to improve the convergence of the dispersion integrals and enhance the validity of the quark-hadron duality assumption \cite{Colangelo:2000dp}. 
% When applying the Borel transformation to Eq.\eqref{equ_dc_Im}, the decay constants $\lambda_{\Lambda_b}^{L,R}$ satisfy
% \begin{equation}{\label{eq:final-result}}
%      \begin{aligned}
%                     \left(\lambda^{L,R}_{\Lambda_b}  \right)^2 & e^{-m_{\Lambda_b}^2/M^2} = \frac{1}{\pi}\int_{m_b^2}^{s_0^{\Lambda_b}}   ds\ e^{-s/M^2}\ \mathbf{Im}~\!\Pi_{\Lambda_b, 0}^{L,R}  \left(s \right)_{OPE},    
%      \end{aligned}
% \end{equation}
% where $M^2$ is the Borel parameter. 
% The dependence of the decay constants $\lambda_{\Lambda_b}$ on the Borel parameter $M^2$ is illustrated in FIG.\ref{fig:decay_constant_lambda_b}. 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.52\textwidth]{Fig/decay-constant-Lambda-b1.eps}
%     \caption{The $M^2$-dependence of $\Lambda_b$ decay constants in different effective threshold $s_0^{\Lambda_b}$.}
%     \label{fig:decay_constant_lambda_b}
% \end{figure}
% Since the Borel parameter $M^2$ is unphysical, we have to identify an optimal windows in which the decay constant does not significantly depend on the Borel parameter. 
% Finally, when setting the effective threshold at $\sqrt{s_0^{\Lambda_b}}= (6.2 \pm 0.1) $ GeV and considering the QCD input parameters\footnote{The values of QCD input parameters are shown in Appendix. \ref{Appen-QCD-input}.}, the value of $\Lambda_b$ decay constant will be given by
% \begin{equation}
%      |\lambda^{L,R}_{\Lambda_b}| = \left( 1.7 \pm 0.1 \pm 0.3 \right) \times 10^{-2}~~[\text{GeV}^3],
% \end{equation}
% where the first uncertainty originates from the uncertainties of the effective threshold $s_0^{\Lambda_b}$ and the Borel parameter $M^2$, while the second one arises from the uncertainties of the QCD input parameters.

  








==> 4-QCD_factorization_in_Baryongenies_model.tex <==
\part{Baryongenies modle}

\begin{figure}[h]
\begin{centering}
\includegraphics[scale=0.35]{Fig/Baryongenies_interaction.eps}
\par\end{centering}
\caption{Baryongenies interaction}
\end{figure}
%
In the Baryongenies new physics model, the Lagrangian describing the
interaction between the dark matter spinor field and the quark field
is:
\begin{equation}
\begin{aligned}\mathcal{L} & =\epsilon^{ijk}y_{ub}Y_{i}^{*}\bar{u}_{j}^{c}b_{k}+\epsilon^{ijk}z_{sb}Z_{i}^{-2/3}\bar{s}_{j}^{c}b_{k}+\epsilon^{ijk}y_{us}Y_{i}\bar{u}_{j}^{c}s_{k}\\
 & +\epsilon^{ijk}z_{db}Z_{i}\bar{d}_{j}^{c}b_{k}+\epsilon^{ijk}z_{ub}Y_{i}^{*}\bar{u}_{j}^{c}b_{k}+\epsilon^{ijk}y_{ud}Y_{i}^{*}\bar{u}_{j}^{c}d_{k}\\
 & +\epsilon^{ijk}y_{\Psi s}Y_{i}\bar{\Psi}_{R}^{c}s_{k,R}+\epsilon^{ijk}Z_{i}^{-2/3*}y_{\Psi u}\bar{\Psi}_{R}^{c}u_{k,R}\\
 & +\epsilon^{ijk}Y_{i}y_{\Psi b}\bar{\Psi}_{R}^{c}b_{k,R}+\epsilon^{ijk}Y_{i}^{*}y_{\Psi d}\bar{\Psi}_{R}^{c}d_{k,R}\\
 & +y_{\phi\xi}\bar{\Psi}\phi\xi+h.c
\end{aligned}
\end{equation}
%
The corresponding diagram for the Lagrangian is depicted in Figure
1. In the decay process of Baryongenies, it can be mediated by exchanging
a heavy new physics particle Y and Z, with charges $Q_{Y}=-1/3e$
and $Q_{Z}=-2/3e$, respectively. Within the framework of effective
field theory, we integrate out the heavy propagators to obtain the
effective Hamiltonian.
%
\begin{equation}
\mathcal{H}_{eff}=\sum_{\alpha=1}^{6}G_{\alpha}O_{\alpha}^{H}
\end{equation}
%
where $G_{\alpha}$ represents the effective coupling constant of
the new physics. In the operator $O_{\alpha}^{H}$ , the superscript
$H$stands for helicity. For the operator $O_{\alpha}^{RR}$, the
leading-twist wave function cannot be projected out. In the following
calculation, we consider the contribution of the $O_{\alpha}^{LR}$
operator, which has the specific form
\begin{equation}
\begin{aligned}O_{1,ubs}^{LR} & =\epsilon^{ijk}(\bar{u}_{i,L}^{c}b_{j,L})(\bar{\Psi}_{R}^{c}s_{k,R})\\
O_{2,sbu}^{LR} & =\epsilon^{ijk}(\bar{s}_{i,L}^{c}b_{j,L})(\bar{\Psi}_{R}^{c}u_{k,R})\\
O_{3,usb}^{LR} & =\epsilon^{ijk}(\bar{u}_{i,L}^{c}s_{j,L})(\bar{\Psi}_{R}^{c}b_{k,R})
\end{aligned}
,\qquad\begin{aligned}O_{4,dbu}^{,LR} & =\epsilon^{ijk}(\bar{d}_{i,L}^{c}b_{j,L})(\bar{\Psi}_{R}^{c}u_{k,R})\\
O_{5,ubd}^{LR} & =\epsilon^{ijk}(\bar{u}_{i,L}^{c}b_{j,L})(\bar{\Psi}_{R}^{c}d_{k,R})\\
O_{6,udb}^{LR} & =\epsilon^{ijk}(\bar{u}_{i,L}^{c}d_{j,L})(\bar{\Psi}_{R}^{c}b_{k,R})
\end{aligned}
\end{equation}
where the superscript $c$ represents the charge conjugation transformation
$\bar{\psi}^{c}=\psi^{T}C$.
%
\part{QCD calculation}
%
In the Baryongenies model, considering the decay of heavy-flavor baryons
into final-state light pseudoscalar mesons and heavy dark matter baryon
fields with masses around 1 GeV, the final-state particles can be
approximately regarded as being on the light cone. Let's denote the
momentum of the final-state mesons or photons as $q$ along the light-cone
direction, and the momentum of the final-state dark matter particles
as $p$ along the anti-light-cone direction. We take the large momentum
as $n\cdot q=\bar{n}\cdot p=m_{\Lambda_{b}}$ for the $\Lambda_{b}$
baryon decay processes, and $n\cdot q=\bar{n}\cdot p=m_{\Xi_{b}}$
for the $\Xi_{b}^{-}$ baryon decay processes. To calculate the decay
amplitude, we need to introduce the definition of the pseudoscalar
meson LCDAs
%
\begin{equation}
\left\langle P(p)|\,[\bar{q}(t\bar{n})]_{A}\,[t\bar{n},0]\,[q(0)]_{B}\,|0\right\rangle =\dfrac{if_{P}}{4}\,\bar{n}\cdot p\,\bigg[\,\dfrac{\slashed{n}}{2}\,\gamma_{5}\,\bigg]_{BA}\int_{0}^{1}dx\,e^{ixt\bar{n}\cdot p}\,\phi_{P}(x,\mu),
\end{equation}
%
where $x$ and $\bar{x}$ represent the momentum fraction of $\bar{q}$
quark and $q$ respectively in mesons, the connection between quarks
is established through the gluon field in gauge theory
%
\begin{equation}
[t\bar{n},0]=\mathrm{P}\,\mathrm{exp}\bigg[\,ig\int_{0}^{t}dx\,\bar{n}\cdot A(x\bar{n})\,\bigg],
\end{equation}
%
The leading-twist LCDAs of pseudoscalar mesons can be expanded using
Gegenbauer polynomials.
%
\begin{equation}
\phi_{P}(x,\mu)=6x(1-x)\bigg[\,1+\sum_{n=1}^{\infty}a_{n}^{P}(\mu)\,C_{n}^{(3/2)}(2x-1)\,\bigg],
\end{equation}
%
the numerical input of pseudoscalar meson are shown in Table 4. 
%
\begin{table} 	
\caption{Imput parameter at $\mu_{0}=1\,\mathrm{GeV}$\label{tab:Input_Para}.} 	
\begin{spacing}{1.8} 		
\noindent \centering{}% 		
\begin{tabular}{ll|ll} 			
\hline 			
\hline  			
$\quad m_{\Lambda_{b}}=5.6196\,\mathrm{GeV}$ & \cite{ParticleDataGroup:2022pth}	& $\quad\tau_{\Lambda_{b}}=1.471\,\mathrm{ps}$ & \cite{ParticleDataGroup:2022pth} \\ 
$\quad m_{\Xi_{b}}=5.7970\,\mathrm{GeV}$ & \cite{ParticleDataGroup:2022pth}	& $\quad\tau_{\Xi_{b}}=?,\mathrm{ps}$ & \cite{ParticleDataGroup:2022pth} \\			%
$\quad\omega_{0}=0.280\,_{-0.038}^{+0.047}\,\mathrm{GeV}$ & \cite{Wang:2015ndk} $\quad$ & 	$\quad f_{\Lambda_{b}}^{(2)}(\mu_{0})=0.030\pm 0.005\,\mathrm{GeV}^{3}$ \quad & \cite{Wang:2015ndk}$\quad$\\ 			
$\quad f_{\pi}=0.1304\pm0.0002\,\mathrm{GeV}$ \quad& \cite{Grossman:2015cak} $\quad$&	$\quad f_{K}=0.1562\pm0.0007\,\mathrm{GeV}$ & \cite{Grossman:2015cak} \\ 		
$\quad a_{1}^{\pi}(\mu_{0})=0$ & \cite{Grossman:2015cak} &	$\quad a_{2}^{\pi}(\mu_{0})=0.29\pm0.08$ & \cite{Grossman:2015cak}\\ 
$\quad a_{1}^{K}(\mu_{0})=-0.07\pm0.04$ & \cite{Grossman:2015cak} $\quad$ &	$\quad a_{2}^{K}(\mu_{0})=0.24\pm0.08$ & \cite{Grossman:2015cak}\\ 
%	
\hline  			
\hline 		
\end{tabular} 	
\end{spacing} 
\end{table} The definition of $\Lambda_{b}$ LCDA is 
%
\begin{equation}
\begin{aligned} 
&\langle 0|\,[u_{i}(t_{1}n)]_{A}\,[0,t_{1}n]\,[d_{j}(t_{2}n)]_{B}\,[0,t_{2}n]\,[h_{v,k}(0)]_{C}\,|\Lambda_{b}(v)\rangle \\
= & \dfrac{\epsilon^{ijk}}{4N_{c}!}\,f_{\Lambda_{b}}^{(2)}(\mu)\,[u_{\Lambda_{b}}(v)]_{C}\,\bigg[\,\dfrac{\slashed{\bar{n}}}{2}\,\gamma_{5}\,C^{T}\,\bigg]_{BA}\int_{0}^{\infty}d\omega\,\omega\int_{0}^{1}du\,e^{-i\omega(t_{1}u+it_{2}\bar{u})}\,\psi_{2}(u,\omega),
\end{aligned}
\end{equation}
%
and $\Xi_{b}$ LCDA is
\begin{equation}
\begin{aligned} 
\,& \langle 0|\,[d_{i}(t_{1}n)]_{A}\,[0,t_{1}n]\,[s_{j}(t_{2}n)]_{B}\,[0,t_{2}n]\,[h_{v,k}(0)]_{C}\,|\Xi_{b}^{-}(v)\rangle \\
= & \dfrac{\epsilon^{ijk}}{4N_{c}!}\,f_{\Xi_{b}}^{(2)}(\mu)\,[u_{\Xi_{b}^{-}}(v)]_{C}\,\bigg[\,\dfrac{\slashed{\bar{n}}}{2}\,\gamma_{5}\,C^{T}\,\bigg]_{BA}\int_{0}^{\infty}d\omega\,\omega\int_{0}^{1}du\,e^{-i\omega(t_{1}u+it_{2}\bar{u})}\,\psi_{2}(u,\omega),
\end{aligned}
\end{equation}
%
similarily, the quarks are connected through the gauge field of the
gluon to maintain gauge invariance
\begin{equation}
[0,t_{i}n]=\mathrm{P}\,\mathrm{exp}\bigg[\,-ig\int_{0}^{t_{i}}dx\,n\cdot A(xn)\,\bigg]
\end{equation}
%
Where $i=1,2$. The definition of the leading-twist wave function
for the $\Lambda_{b}$ baryon is given by
\begin{equation}
\psi_{2}(u,\omega)=u\,(1-u)\,\omega^{2}\,\dfrac{1}{\omega_{0}^{4}}\,e^{-\omega/\omega_{0}},
\end{equation}
%
In SU(3) symmetry, the LCDA of the $\Xi_{b}$ baryon is consistent
with that of the $\Lambda_{b}$ one , therefore we adopt the same
form of wave function input parameters of $\omega_{0}$.
%
\part{Spectator processes }
%
\section{$\Lambda_{b}\rightarrow P\Psi$ form factor in QCD}
%
\begin{figure}
\begin{centering}
\includegraphics[scale=0.4]{Fig/Lambda_b_P_Psi.eps}
\par\end{centering}
\caption{Paragraph in the \textsf{Abstract} environment}
\end{figure}

For the $\Lambda_{b}$ decay processes, the operators $O_{1}^{LR}\sim O_{3}^{LR}$
represent $\Lambda_{b}\rightarrow K^{0}\Psi$ decay processes and
the operators $O_{4}^{LR}\sim O_{6}^{LR}$ represents $\Lambda_{b}\rightarrow\pi^{0}\Psi$
processes. For the $\Xi_{b}^{-}$ decay processes, the operators $O_{1}^{LR}\sim O_{3}^{LR}$
represent $\Xi_{b}^{-}\rightarrow K^{-}\Psi$ decay processes and
the operators $O_{4}^{LR}\sim O_{6}^{LR}$ represents $\Xi_{b}^{-}\rightarrow\pi^{-}\Psi$
decay processes. According to reference {[}{]}, we employ the method
of QCD factorization to expand the decay amplitude to leading power
and perform factorization analysis. The decay amplitude in the leading
power case is given by:
\begin{equation}
\begin{aligned}\mathcal{A}_{\Lambda_{b}\rightarrow P^{0}\Psi,\alpha} & =\zeta_{\Lambda_{b}\rightarrow P^{0},\alpha}\times v_{\Psi}^{T}(q)M_{\Lambda_{b}\rightarrow P^{0},\alpha}u_{\Lambda_{b}}(v)\\
\mathcal{A}_{\Xi_{b}^{-}\rightarrow P^{-}\Psi,\alpha} & =\zeta_{\Xi_{b}^{-}\rightarrow P^{-},\alpha}\times v_{\Psi}^{T}(q)M_{\Xi_{b}^{-}\rightarrow P^{-},\alpha}u_{\Xi_{b}^{-}}(v)
\end{aligned}
\end{equation}
%
Since the initial heavy baryon fields and the final dark heavy baryon
fields are both spinor fields, the decay amplitude is also composed
of spinor structures. The matrix elements of different operators are:
\begin{equation}
\begin{aligned} & M_{\Lambda_{b}\rightarrow\pi^{0},1}=-M_{\Lambda_{b}\rightarrow\pi^{0},2}=M_{\Lambda_{b}\rightarrow K^{0},4}/\sqrt{2}=-M_{\Lambda_{b}\rightarrow K^{0},5}/\sqrt{2}=-\sqrt{2}m_{\Lambda_{b}}^{1/2}\bar{n}\cdot p\,CP_{R}\dfrac{\slashed{n}}{2}\\
 & M_{\Xi_{b}^{-}\rightarrow K^{-},1}=-M_{\Xi_{b}^{-}\rightarrow K^{-},2}=-M_{\Xi_{b}^{-}\rightarrow\pi^{-},2}=-M_{\Xi_{b}^{-}\rightarrow\pi^{-},2}=-2m_{\Xi_{b}^{-}}^{1/2}\bar{n}\cdot p\,CP_{R}\dfrac{\slashed{n}}{2}
\end{aligned}
\end{equation}
%
The specific form of the form factor is given by
%
\begin{equation}
\begin{aligned}\zeta_{\Lambda_{b}\rightarrow P^{0},\alpha} & =f_{P}f_{\Lambda_{b}}^{(2)}\int_{0}^{\infty}d\omega\omega\int_{0}^{1}du\int_{0}^{1}dx\,C_{\Lambda_{b}\rightarrow P^{0},\alpha}(x,u,\omega,\mu)\mathcal{J}_{\Lambda_{b}\rightarrow P^{0},\alpha}(x,u,\omega,\mu)\phi_{P}(x)\psi_{2}(u,\omega)\\
\zeta_{\Xi_{b}^{-}\rightarrow P^{-},\alpha} & =f_{P}f_{\Xi_{b}}^{(2)}\int_{0}^{\infty}d\omega\omega\int_{0}^{1}du\int_{0}^{1}dx\,C_{\Xi_{b}^{-}\rightarrow P^{-},\alpha}(x,u,\omega,\mu)\mathcal{J}_{\Xi_{b}^{-}\rightarrow P^{-},\alpha}(x,u,\omega,\mu)\phi_{P}(x)\psi_{2}(u,\omega)
\end{aligned}
\end{equation}
%
where $C$ is the hard function with $C=1$ at the tree level and the jet-function is 
\begin{equation}
\begin{aligned}\mathcal{J}_{\Lambda_{b}\rightarrow\pi^{0},\alpha}(x,u,\omega,\mu) & =\dfrac{\pi\alpha_{s}(\mu)T_{\Lambda_{b}\rightarrow\pi^{0},\alpha}}{4\bar{n}\cdot p}\bigg(\dfrac{1}{\bar{u}\omega^{2}x}+\dfrac{1}{u\omega^{2}x}\bigg),\qquad\alpha=1\sim2\\
\mathcal{J}_{\Lambda_{b}\rightarrow K^{0},\alpha}(x,u,\omega,\mu) & =\dfrac{\pi\alpha_{s}(\mu)T_{\Lambda_{b}\rightarrow K^{0},\alpha}}{4\bar{n}\cdot p}\dfrac{1}{\bar{u}\omega^{2}x},\qquad\alpha=4\sim5\\
\mathcal{J}_{\Xi_{b}^{-}\rightarrow K^{-},\alpha}(x,u,\omega,\mu) & =\dfrac{\pi\alpha_{s}(\mu)T_{\Xi_{b}^{-}\rightarrow K^{-},\alpha}^{a}}{4\bar{n}\cdot p}\dfrac{1}{\bar{u}\omega^{2}x},\qquad\alpha=1\sim2\\
\mathcal{J}_{\Xi_{b}^{-}\rightarrow\pi^{-},\alpha}(x,u,\omega,\mu) & =\dfrac{\pi\alpha_{s}(\mu)T_{\Xi_{b}^{-}\rightarrow\pi^{-},\alpha}^{a}}{4\bar{n}\cdot p}\dfrac{1}{u\omega^{2}x},\qquad\alpha=4\sim5
\end{aligned}
\end{equation}
%
where the color factors for the non-zero terms are 
\begin{equation}
\begin{aligned}T_{\Lambda_{b}\rightarrow\pi^{0},1} & =-T_{\Lambda_{b}\rightarrow\pi^{0},2}=-T_{\Lambda_{b}\rightarrow K^{0},4}=T_{\Lambda_{b}\rightarrow K^{0},5}=-\dfrac{2}{9}\\
T_{\Xi_{b}^{-}\rightarrow\pi^{-},1} & =-T_{\Xi_{b}^{-}\rightarrow\pi^{-},2}=-T_{\Xi_{b}^{-}\rightarrow K^{-},4}=-T_{\Xi_{b}^{-}\rightarrow\pi^{-},5}=\dfrac{2}{9}
\end{aligned}
\end{equation}
In Eq. (), $\phi(x)$ and $\psi(u,\omega)$ respectively represent
the nonperturbative meson and baryon wave functions, representing
the nonperturbative effects of the decay process. It can be observed
that the short-distance behavior of the jet function can be absorbed
by the wave functions, allowing for factorization without endpoint
divergence.


\section{Radiatived decay}
%
\begin{figure}
\begin{centering}
\includegraphics[scale=0.4]{Fig/Lambda_b_to_gamma_l.eps}
\par\end{centering}
\caption{Paragraph in the environment}
\end{figure}
%
For the Radiatived decay processes, only the operators $O_{1}^{LR}\sim O_{3}^{LR}$
will contribute to $\Lambda_{b}\rightarrow\gamma\Psi$ leadingn power
decay processes. Accroding Ref., we use the QCD factorization framework,
the leading power decay amplitudes are 
%
\begin{equation}
\mathcal{A}_{\Lambda_{b}\rightarrow\gamma\Psi,\alpha}=\zeta_{\Lambda_{b}\rightarrow\gamma,\alpha}\times v_{\Psi}^{T}(q)M_{\Lambda_{b}\rightarrow\gamma,\alpha}u_{\Lambda_{b}}(v)
\end{equation}
%
where the matrix elements of different operators are:
\begin{equation}
M_{\Lambda_{b}\rightarrow\gamma,\alpha}=m_{\Lambda_{b}}^{1/2}\bar{n}\cdot p\,CP_{R}\dfrac{\slashed{n}}{2}\dfrac{\slashed{\bar{n}}}{2}\slashed{\epsilon}_{\perp},\qquad\alpha=1\sim3
\end{equation}
%
Since photons can radiate from different light quark lines, in the
leading power scenario, there will be contributions from two diagrams.
Therefore, the operator $O_{3}$ 
\begin{equation}
\zeta_{\Lambda_{b}\rightarrow\gamma,\alpha}=f_{\Lambda_{b}}^{(2)}\int_{0}^{\infty}d\omega\omega\int_{0}^{1}du\mathcal{J}_{\Lambda_{b}\rightarrow\gamma,\alpha}(x,u,\omega,\mu)\psi_{2}(u,\omega)
\end{equation}
%
The jet functions in foem factors are
\begin{equation}
\begin{aligned}\mathcal{J}_{\Lambda_{b}\rightarrow\gamma,\alpha}(x,u,\omega,\mu) & =\dfrac{T_{\Lambda_{b}\rightarrow\gamma,\alpha}}{4}\bigg(\dfrac{Q_{u}}{u\omega}-\dfrac{Q_{d}}{\bar{u}\omega}\bigg),\qquad\alpha=1\\
\mathcal{J}_{\Lambda_{b}\rightarrow\gamma,\alpha}(x,u,\omega,\mu) & =\dfrac{T_{\Lambda_{b}\rightarrow\gamma,\alpha}}{4}\dfrac{Q_{d}}{\bar{u}\omega},\qquad\alpha=2\sim3
\end{aligned}
\end{equation}
%
In the expression, the electric charges of the light quarks $u$ and
$d$ are respectively $Q_{u}=2/3e$ and $Q_{u}=-1/3e$. The color
factors are
\begin{equation}
\begin{aligned}T_{\Lambda_{b}\rightarrow\gamma,1} & =-T_{\Lambda_{b}\rightarrow\gamma,1}=-T_{\Lambda_{b}\rightarrow\gamma,1}=1\end{aligned}
\end{equation}


\section{Numerical result}
%
In this section, we perform numerical calculations based on the form
factors obtained in the previous section. We choose the QCD and QED
coupling constants as $\alpha_{s}(\mu=2GeV)=0.3$ and $\alpha_{em}(\mu=2GeV)=1/137$.
According to the results in the table, we can compute the form factors
for the decay process within the Baryongenies model. The numerical
result for the form factor of the spectator processes $\Lambda_{b}\rightarrow P^{0}\Psi$
are
%
\begin{equation}
\begin{aligned}|\zeta_{\Lambda_{b}\rightarrow\pi^{0},\alpha}| & =1.80\,_{-0.68}^{+0.58}\times10^{-3}\,\mathrm{GeV},\qquad\alpha=1\sim2,\\
|\zeta_{\Lambda_{b}\rightarrow K^{0},\alpha}| & =1.09\,_{-0.42}^{+0.36}\times10^{-3}\,\mathrm{GeV},\qquad\alpha=4\sim5.
\end{aligned}
\end{equation}
%
The numerical result for the form factor of the spectator processes
$\Xi_{b}^{-}\rightarrow P^{-}\Psi$ are
%
\begin{equation}
\begin{aligned}|\zeta_{\Xi_{b}^{-}\rightarrow K^{-},\alpha}| & =1.11\,_{-0.40}^{+0.34}\times10^{-3}\,\mathrm{GeV},\qquad\alpha=1\sim2\\
|\zeta_{\Xi_{b}^{-}\rightarrow\pi^{-},\alpha}| & =1.70\,_{-0.66}^{+0.57}\times10^{-3}\,\mathrm{GeV},\qquad\alpha=4\sim5
\end{aligned}
\end{equation}
%
The numerical result for the form factor of the spectator processes
$\Lambda_{b}\rightarrow\gamma\Psi$ are

\begin{equation}
\begin{aligned}|\zeta_{\Lambda_{b}\rightarrow\gamma,\alpha}| & =8.11\,_{-1.92}^{+1.74}\times10^{-3}\,\mathrm{GeV},\qquad\alpha=1\\
|\zeta_{\Lambda_{b}\rightarrow\gamma,\alpha}| & =2.70\,_{-0.64}^{+0.58}\times10^{-3}\,\mathrm{GeV},\qquad\alpha=2\sim3
\end{aligned}
\end{equation}
%
The square of the matrix element with spinor structure of the decay
amplitude is proportional to:
%
\begin{equation}
   \begin{aligned}|\mathcal{A}_{\Xi_{b}^{-}\rightarrow P^{-}\Psi,\alpha}|^{2} & \sim|\zeta_{\Xi_{b}^{-}\rightarrow P^{-},\alpha}|^{2}\times\mathrm{Tr}\bigg\{(\slashed{q}-m_{\Psi})^{T}CP_{R}\dfrac{\slashed{n}}{2}(\slashed{v}+1)\dfrac{\slashed{n}}{2}P_{L}C\bigg\}\\
 & \sim|\zeta_{\Xi_{b}^{-}\rightarrow P^{-},\alpha}|^{2}\times\mathrm{Tr}\bigg\{ Cn\cdot q\dfrac{\slashed{\bar{n}}}{2}CCP_{R}\dfrac{\slashed{n}}{2}\dfrac{\slashed{n}}{2}\dfrac{\slashed{n}}{2}P_{L}C\bigg\}\\
 & \sim|\zeta_{\Xi_{b}^{-}\rightarrow P^{-},\alpha}|^{2}\times n\cdot q
\end{aligned}
\end{equation}
%
For ease of calculation, we provide the amplitude as follows. $\Lambda_{b}\rightarrow P^{0}\Psi$
processes are
%
\begin{equation}
\begin{aligned}|\mathcal{A}_{\Lambda_{b}\rightarrow\pi^{0}\Psi,1}|^{2} & =G_{new,1}\times2m_{\Lambda_{b}}^{4}\times|\zeta_{\Lambda_{b}\rightarrow\pi^{0},1}|^{2}\\
|\mathcal{A}_{\Lambda_{b}\rightarrow\pi^{0}\Psi,2}|^{2} & =G_{new,2}\times2m_{\Lambda_{b}}^{4}\times|\zeta_{\Lambda_{b}\rightarrow\pi^{0},2}|^{2}\\
|\mathcal{A}_{\Lambda_{b}\rightarrow\pi^{0}\Psi,3}|^{2} & =0\\
|\mathcal{A}_{\Lambda_{b}\rightarrow K^{0}\Psi,4}|^{2} & =G_{new,4}\times4m_{\Lambda_{b}}^{4}\times|\zeta_{\Lambda_{b}\rightarrow K^{0},4}|^{2}\\
|\mathcal{A}_{\Lambda_{b}\rightarrow K^{0}\Psi,5}|^{2} & =G_{new,5}\times4m_{\Lambda_{b}}^{4}\times|\zeta_{\Lambda_{b}\rightarrow K^{0},5}|^{2}\\
|\mathcal{A}_{\Lambda_{b}\rightarrow K^{0}\Psi,6}|^{2} & =0
\end{aligned}
\end{equation}
%
$\Xi_{b}^{-}\rightarrow P^{-}\Psi$ processes are
%
\begin{equation}
\begin{aligned}|\mathcal{A}_{\Xi_{b}^{-}\rightarrow K^{-}\Psi,1}|^{2} & =G_{new,1}\times4m_{\Xi_{b}}^{4}\times|\zeta_{\Xi_{b}^{-}\rightarrow K^{-},1}|^{2}\\
|\mathcal{A}_{\Xi_{b}^{-}\rightarrow K^{-}\Psi,2}|^{2} & =G_{new,2}\times4m_{\Xi_{b}}^{4}\times|\zeta_{\Xi_{b}^{-}\rightarrow K^{-},2}|^{2}\\
|\mathcal{A}_{\Xi_{b}^{-}\rightarrow K^{-}\Psi,3}|^{2} & =0\\
|\mathcal{A}_{\Xi_{b}^{-}\rightarrow\pi^{-}\Psi,4}|^{2} & =G_{new,4}\times4m_{\Xi_{b}}^{4}\times|\zeta_{\Xi_{b}^{-}\rightarrow\pi^{-},4}|^{2}\\
|\mathcal{A}_{\Xi_{b}^{-}\rightarrow\pi^{-}\Psi,5}|^{2} & =G_{new,5}\times4m_{\Xi_{b}}^{4}\times|\zeta_{\Xi_{b}^{-}\rightarrow\pi^{-},5}|^{2}\\
|\mathcal{A}_{\Xi_{b}^{-}\rightarrow\pi^{-}\Psi,6}|^{2} & =0
\end{aligned}
\end{equation}
%
$\Lambda_{b}\rightarrow\gamma\Psi$ processes are
%
\begin{equation}
\begin{aligned}|\mathcal{A}_{\Lambda_{b}\rightarrow\gamma,1}|^{2} & =G_{new,1}\times2m_{\Lambda_{b}}^{3}\times|\zeta_{\Xi_{b}^{-}\rightarrow P^{-},1}|^{2}\\
|\mathcal{A}_{\Lambda_{b}\rightarrow\gamma,2}|^{2} & =G_{new,2}\times2m_{\Lambda_{b}}^{3}\times|\zeta_{\Xi_{b}^{-}\rightarrow P^{-},2}|^{2}\\
|\mathcal{A}_{\Lambda_{b}\rightarrow\gamma,3}|^{2} & =G_{new,3}\times2m_{\Lambda_{b}}^{3}\times|\zeta_{\Xi_{b}^{-}\rightarrow P^{-},3}|^{2}
\end{aligned}
\end{equation}

==> 5-Constraint.tex <==
\section{Probe B-Mesogenesis with invisible and semi-invisible decay of bottom baryons}
\label{sec:constraint-for-coupling}

With the hadronic matrix elements obtained in the above section, we can explore the B -Mesogenesis via the  invisible and semi-invisible decays of bottom baryons at the future lepton colliders. 
The reconstructions of the invisible and semi-invisible decays of bottom baryons are always difficult in experiments. But it can be overcome by the double tag method \cite{MARK-III:1989dea}. 
In the $e^+e^-$ collisions, the initial energy is well known in each event.  
Suppose a good resolution in the detectors, we reconstruct all the recoiling particles except for $\Lambda_b^0/\Xi_b^{0,-}$ in the colliding event, which helps to determine the invariant mass of the bottom-baryon candidate using the energy-momentum conservation. 
It would be identified as a production of bottom baryon, if the invariant mass is consistent with the mass of $\Lambda_b^0/\Xi_b^{0,-}$ and the conservation laws are satisfied for the electric charge, the baryon number, the bottom number and the strange number. 
Then we are able to measure the invisible and semi-invisible decays of bottom baryons. 
The double tag method has been widely used by BESIII, BABAR and Belle. For example, BESIII measured the absolute branching fraction of $\Lambda_c^+\to \Lambda^0e^+\nu_e$ at the $\Lambda_c^+\bar\Lambda_c^-$ threshold, which determines $\Lambda_c^+$ by reconstructing the charmed anti-baryon via its hadronic decays such as $\bar\Lambda_c^-\to \bar p K^+\pi^-$ \cite{BESIII:2015ysy}. 
It is also possible to use the double tag method at the energy much higher than the baryon-antibaryon threshold.  
The Belle collaboration measured the absolute branching fractions of $\Lambda_c^+$ decays with reconstructing the recoiling $D^{(*)-}\bar p\pi^+$ system in the event of  $e^+e^-\to D^{(*)-}\bar p\pi^+\Lambda_c^+$ at the colliding energy around 10 GeV \cite{Belle:2013jfq}. 
Therefore, the invisible and semi-invisible decays of $\Lambda_b^0/\Xi_b^-$ can be measured using the double tag method at the $e^+e^-$ colliders, such as BelleII at the bottom baryon-antibaryon threshold, or CEPC and FCC-ee at a higher energy as well. 

In practice to estimate the sensitivity on the parameters of B-Mesogenesis, we define the significance $s$ of the signal at $95\%$ C.L. as
\begin{equation}
s=\frac{n_S}{\sqrt{n_S+n_B}}
=\sqrt{n_S}=\sqrt{N_{\mathcal{B}}\times Br(\mathcal{B}\to X)}
=2,
\end{equation}
where $n_S$, $n_B$ denote the events number of signal and background at future lepton colliders. 
The background events are negligible using the double tag method, since the three kinds of processes studied in this work are all forbidden in the Standard Model by the visible baryon number violation.  
The branching fractions  $Br(\mathcal{B}\to X)$ with $X=\pi\bar{\psi}, K\bar{\psi}, \gamma\bar{\psi}, \xi\bar{\phi}$ are given in Eqs. (\ref{equ:BRmeson},\ref{equ:BRgamma},\ref{eq_branching-ratio}), respectively.
$N_\mathcal{B}$ represents the production number of bottom baryons detected by the double tag method.
Notice its difference from the total production of bottom baryons in the collisions.
Besides, we assume an efficiency of  reconstruction as $100\%$  for pion, kaon and photon in the semi-invisible decays. 
In this work, we assume the production number of bottom baryons by the double tag method are $N_\mathcal{B}=N_{\Lambda_b,\Xi_b}=10^8$ as a benchmark for the future lepton colliders. 
The corresponding constraints can directly scale up to the results respected to the actual production number of bottom baryons at future lepton colliders, which are still indistinct in the current theoretical study.

%since proton's life-time is tightly constraints by SNO+ measurement \cite{SNO:2022trz}, 
There are some constraints on the masses of the dark particles under the B-Mesogenesis scenario. 
To prevent the decay of proton into the dark fermion, the mass of dark fermion $m_\psi$ must satisfy
\begin{equation}
    m_{\psi} > m_p -m_e  \simeq 937.8\; \text{MeV}.
\end{equation} 
In addition, the stability of dark matter requires the mass difference between the dark scalar $\phi$ and dark Majorana fermion $\xi$ must obey \cite{Alonso-Alvarez:2021qfd}
\begin{equation}{\label{equ_mass_splitting}}
    |m_{\xi}- m_{\phi}| < m_p + m_e \simeq 938.8\ \text{MeV}.
\end{equation}



 
\subsection{Probe B-Mesogenesis in semi-invisible decays of bottom baryons.}


Firstly, we estimate the sensitivity on the B-Mesogenesis by searching for the semi-invisible decay of bottom baryons at future lepton colliders. Their branching ratios are only sensitive to the mass $m_\psi$ and Wilson coefficients $|C^L_{ub,d}|$ or $|C^L_{ub,s}|$ of the scenario. 
%
The constraints on the Wilson coefficients $|C^L_{ub,d}|$ and $|C^L_{ub,s}|$ versus $m_\psi$ at $95\%$ C.L. are illustrated in FIG. \ref{fig:constraint-Wilson-coefficient}, where the production number of bottom baryons by the double tag method are assuming to be $N_{\Lambda_b,\Xi_b}=10^8$. 
The constraints on the right-handed operators $\mathcal{O}^R_{ud_a,d_b}$ are omitted as they could not project out the leading-twist wave function of $\Lambda_b$ and $\Xi_b$ baryons. 

\begin{figure}{}
    \centering
    \!\!\subfigure[]{\includegraphics[width=0.48\textwidth]{Fig/Constraint-ubd.eps}} 
    \subfigure[]{\includegraphics[width=0.48\textwidth]{Fig/Constraint-ubs.eps}}
    \caption{The constraints on the Wilson coefficients at $95\%$ C.L. versus $m_\psi$ in the semi-invisible decays of bottom baryons.
    The left panel illustrates the constraints on $|C^L_{ub,d}|$, while the right panel display the constraints on $|C^L_{ub,s}|$.
    The enhancements at the large mass region arise from the evolution of form factor. 
    The declines of the constraints at the tail result from the suppression of phase space.
    When dark fermion mass $m_\psi$ close to the mass of $\Lambda_b^0$ baryon, the soft photon radiation in $\Lambda_b^0\to\gamma\bar{\psi}$ channel will induce a serious infrared divergence, which invalid the leading order estimation in this region.
    Hence, we omit the constraints in $\Lambda_b^0\to\gamma\bar{\psi}$ process when $m_\psi>5$ GeV (blue dot dashed line).
}
    \label{fig:constraint-Wilson-coefficient}
\end{figure}



For $\Lambda_b(\Xi_b)\to P\bar{\psi}$ processes, we found that the semi-invisible decay $\Lambda_b^0\to\pi^0\bar{\psi}$ is most sensitive to operator $\mathcal{O}^L_{ub,d}$, while the $\Xi^-_b\to \pi^-\bar{\psi}$ process is most sensitive to operator $\mathcal{O}^L_{ub,s}$. 
When assuming the production number of bottom baryons by the double tag method is $N_{\Lambda_b,\Xi_b}=10^8$, the constraints on the Wilson coefficient can reach $\mathcal{O}(10^{-8})$ GeV$^{-2}$.  
%{\color{blue}{(are given by $|C^L_{ub,d}|\leq3.9\times10^{-8}$ GeV$^{-2}$ and $|C^L_{ub,s}|\leq4.3\times10^{-8}$ GeV$^{-2}$)}}.
The enhancements of the constraints at the large mass region arise from the evolution of form factors. 
And the declines of the Wilson coefficients at the tail result from the suppression of phase space. 
Note that the form factors and the hadrons mass in semi-invisible decay are similar, the constraints on the Wilson coefficients are adjacent in these processes. 

For the $\Lambda_b^0\to\gamma\bar{\psi}$ channel, the constraints on the Wilson coefficients is $\mathcal{O}(10^{-7})$ GeV$^{-2}$.
%given by $|C^L_{ub,d}|\leq1.5\times10^{-7}$ GeV$^{-2}$. 
This constraint is looser than that in the hadronic semi-invisible decay, 
due to the form factors of photon radiation is smaller than those of meson final states.
What's more, when the dark fermion mass $m_\psi$ close to the mass of initial baryons $m_{\Lambda_b}$, the divergence in the evolution of form factors invalid the estimation of branching ratio. 
Therefore, we omit the constraints in $\Lambda_b^0\to\gamma\bar{\psi}$ channel when $m_\psi>5$ GeV.



Last but not least, since the final state hadrons in $\Xi_b^-$ semi-invisible decay are all electric charged, these decay modes could be probed at higher energy future lepton colliders (i.e. CEPC or FCC-ee) with a displaced vertex method. 
Therefore, we expect a well exploration on these semi-invisible decay of bottom baryons at future lepton colliders.









\subsection{Probe B-Mesogenesis in invisible decay of bottom baryons.}

As shown in Ref. \cite{Elor:2018twp,Elor:2022jxy,Khodjamirian:2022vta,Boushmelev:2023huu,Shi:2023riy,Shi:2024uqs}, previous studies mainly focus on searching for the dark fermion $\psi$ in the semi-invisible decay of bottom baryons or mesons. 
To keep the dark matter to be stable, the B-Mesogenesis must involve a dark Majorana fermion $\xi$ and a dark scalar baryon $\phi$ and requires all the dark fermion $\psi$ completely decay into these two invisible particles, with $\mathcal{BR}(\psi\to \phi\xi)=100\%$.
Therefore, the coupling of $y_d$ and the interaction of $\bar\psi\phi\xi$ are very hard to be explored in the semi-invisible decays where $\psi$ is always on shell. 
The width of $\psi$ depending on $y_d$ cannot be measured in experiments since the final states $\phi$ and $\xi$ are not measurable.
On the contrary, the $\bar\psi$ is off-shell in the fully invisible decay of $\Lambda_b^0\to\xi\bar{\phi}$, seen in FIG. \ref{fig:model}(i) or FIG. \ref{FIG:Lambda_b_to_invisible}. Then it is able to explore the stable dark matters $\xi$ or $\bar\phi$, and measure the interaction of $y_d\bar\psi\phi\xi$ as shown in the branching fraction of $\Lambda_b^0\to\xi\bar{\phi}$ in Eq. (\ref{eq_branching-ratio}).
So we suggest that the fully invisible decay of $\Lambda_b^0\to\xi\bar{\phi}$ is crucial for probing the B-Mesogeneisis as it provides a distinctive signal to examine the stable dark particles in this scenario.


Assuming the production number of $\Lambda_b^0$ baryon using the double-tag method as $N_{\Lambda_b}=10^8$, the constraints on the parameters $|y_d~\!C^{L,R}_{ud_a,d_b}|$ can be given straightforwardly from Eq. (\ref{eq_branching-ratio}), depending on the different masses of $\bar\psi$, $\bar\phi$ and $\xi$. 
The constraints 
with $95\%$ C.L. are displayed in FIG. \ref{fig:constraint-mchi} and \ref{fig:constraint-Wilson-coefficient-invisible}, for the variations of $m_{\psi}$ and $m_{\xi}+m_{\phi}$, respectively. 

In FIG. \ref{fig:constraint-mchi}, the constraints of the parameters depending on $m_{\psi}$ are given for $|y_d~\!C_{ud,b}^{L,R}|$ in the left panel, and for $|y_d~\!C_{ub,d}^{L,R}|$ in the right panel. 
Three cases of masses of $\xi$ and $\phi$ are shown in the blue, green and red curves, with (i) $m_{\xi}=m_{\phi}=0.4m_{\psi}$, (ii) $m_\xi=0.7m_\psi$, $m_\phi=0.1m_\psi$, and (iii) $m_\xi=0.1m_\psi$, $m_\phi=0.7m_\psi$.
Since the DM stability in Eq. \eqref{equ_mass_splitting} prohibits a large mass difference between dark fermion $\xi$ and dark scalar baryon $\phi$, it imposes a truncation at the large mass region with the specific mass distribution.
We found that the constraints on the parameters of B-Mesogenesis can reach $\mathcal{O}(10^{-7})$ GeV$^{-2}$. 
Since the values of form factors arose from the left- and right-handed operators are the same except for a different sign, the constraints on the operators with different chirality are equal to each other. 
For the operators with different flavour structures, a factor of $2$ in the constraint on $|y_d~\!C^{L,R}_{ub,d}|$ arises from the half suppression of the decay constants $\lambda^{L,R}_{ub,d}$ in the comparison between Eqs.\eqref{equ:InvisibleDecayConstant} and \eqref{equ:InvisibleDecayConstant2}. 
In the mass region which satisfies the DM stability, the constraints on the Wilson coefficients with different mass distribution are similar, even one of the stable particles carry most of the $\bar{\psi}$ mass.
The drop of the constraints at $m_\psi$ close to $m_{\Lambda_b}$ arises from a nearly on-shell transition of $\Lambda_b^0\to\bar{\psi}$, which significantly enlarge the invisible decay rate. 


Similarly, the constraints of parameters  on the mass of $m_{\xi\phi}=m_\xi+m_\phi$ is shown in FIG. \ref{fig:constraint-Wilson-coefficient-invisible}, for $|y_d~\!C^{L,R}_{ud,b}|$ and $|y_d~\!C^{L,R}_{ub,d}|$ in the left and right panels, respectively.
The three cases of (i) $m_\phi=m_\xi$, (ii) $m_\xi=m_\phi+0.9$ GeV, and (iii) $m_\phi=m_\xi+0.9$ GeV, are displayed in blue, green and red curves, respectively, with the mass of $\psi$ fixed as 4.0 GeV. 
It is interesting that the curves are roughly flat at the region of $m_{\xi\phi}$ between 1 GeV and 5 GeV. 
Furthermore, the differences  between the three curves in each figure are also very small. 
These phenomenons indicate that the constraints on the parameters are insensitive to the mass distribution of $m_\xi$ and $m_\phi$. 
This is beneficial to search for the stable particles in B-Mesogenesis. 
If there is a deviation in the semi-invisible decays of bottom baryons or mesons, the fully invisible decay of $\Lambda_b^0$ can further explore the 
stable components which is inherent in B-Mesogenesis.
The declines of the constraints at the large mass region result from the suppression of phase space.





\begin{figure}
    \centering
    \subfigure[]{
\includegraphics[width=0.46\textwidth]{Fig/Constraint-udb-invisible1.eps}}
    ~~\subfigure[]{\includegraphics[width=0.46
\textwidth]{Fig/Constraint-ubd-invisible1.eps}} 
\caption{The constraints on the parameters $|y_d~\!C^{L,R}_{ud,b}|$ and $|y_d~\!C^{L,R}_{ub,d}|$ versus $m_{\psi}$ from the invisible decay of $\Lambda_b^0$ with $95\%$ C.L. We estimate the constraints in three different mass distribution of dark matters.
The left and right panels illustrate the constraints related to operators $\mathcal{O}_{ud,b}^{L,R}$ and $\mathcal{O}_{ub,d}^{L,R}$, respectively.  
The dark matter (DM) stability in Eq. \eqref{equ_mass_splitting} prohibits a large mass difference between dark fermion $\xi$ and dark scalar $\bar{\phi}$, which imposes a truncation at large mass region in the first two distributions (red and green lines).}
    \label{fig:constraint-mchi}
\end{figure}




\begin{figure}{}
    \centering
    \!\!\subfigure[]{\includegraphics[width=0.45\textwidth]{Fig/Constraint-udb-invisible.eps}} 
    \subfigure[]{\includegraphics[width=0.45\textwidth]{Fig/Constraint-ubd-invisible.eps}}
    \caption{ The constraints on the parameters $|y_d~\!C^{L,R}_{ud,b}|$ and $|y_d~\!C^{L,R}_{ub,d}|$ versus total mass $m_{\xi\phi}=m_\xi+m_\phi$ with $95\%$ C.L..
    As the DM stability prohibits a large mass splitting of dark fermion and dark baryons, we estimate the constraints in three different mass distribution of dark matters.
    }
    \label{fig:constraint-Wilson-coefficient-invisible}
\end{figure}






==> 6-Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

The similar densities of baryons and dark matter in the universe imply that they might arise from a same UV complete model. 
The B-Mesogensis, which assume dark matter can be charged under the baryon number, attempts to simultaneously explain the origins of dark matter and baryon asymmetry. 
Most of previous studies mainly concentrate on exploring the semi-invisible decays of $B$ mesons, since this model was proposed.
Actually, the invisible and semi-invisible decays of bottom baryons are also crucial for exploring the B-Mesogenesis at the GeV scale. 
In particular, as the B-Mesogenesis must involves a dark Majorana fermion and a dark scalar baryon to keep the DM and baryon asymmetry stable, the fully invisible decay of $\Lambda_b^0$ yield a distinctive signal to directly probe the stable particles of this scenario. 
What's more, when exploring the B-Mesogenesis in the decays of bottom baryons, the hadronic matrix elements are inevitable and vital for determining the physical observables. 
%In practice, since the matrix elements relate to the strong interaction, we have to utilize a perturbative or non-perturbative method to determine the matrix elements of bottom baryons.
We systematically study the hadronic semi-invisible decays of $\Lambda_b^0\to \pi^0(K^0)\bar\psi$ and $\Xi_b^-\to \pi^-(K^-)\bar\psi$, the radiative semi-invisible decay of $\Lambda_b^0\to \gamma\bar\psi$, and the fully invisible decay of $\Lambda_b^0\to \xi\bar\phi$. The relevant hadronic matrix elements are calculated within the QCD factorization method in the heavy quark limit. 
Finally, we analyze the sensitivities on the parameters of B-Mesogenesis by searching for the invisible and semi-invisible decay of bottom baryons at future lepton colliders.
Assuming the production of bottom baryons by the double-tag method $N_{\Lambda_b,\Xi_b}=10^8$, we found that the constraints on the Wilson coefficients $|C^{L}_{ub,d}|$ and $|C^{L}_{ub,s}|$ in semi-invisible decay of bottom baryons can reach $\mathcal{O}(10^{-8})$ GeV$^{-2}$, while the constraints on $|y_d~\!C^{L,R}_{ud,b}|$ and $|y_d~\!C^{L,R}_{ub,d}|$ can reach $\mathcal{O}(10^{-7})$ GeV$^{-2}$ from the fully invisible decay of $\Lambda_b^0$. 
Although the invisible decay of $\Lambda_b^0$ baryon sensitive to more new physics parameters, we want to emphasize that this decay mode provides a distinctive signal to directly explore the stable dark particles of B-Mesogenesis. 







==> 7-Acknowledgments.tex <==
\section{Acknowledgments}
We are grateful to Sheng-Qi Zhang and Man-Qi Ruan for useful discussions. The work is partly supported by the National Natural Science Foundation of China with Grant No.12335003, 12275277 and the National Key Research and Development Program of China under Contract No.2020YFA0406400 and 2023YFA1606000.
